Scaling Deep Learning Computation over the Inter-Core Connected Intelligence Processor with T10

As AI chips incorporate numerous parallelized cores to scale deep learning (DL) computing, inter-core communication is enabled recently by employing high-bandwidth and low-latency interconnect links on the chip (e.g., Graphcore IPU). It allows each core to directly access the fast scratchpad memory in other cores, which enables new parallel computing paradigms. However, without proper support for the scalable inter-core connections in current DL compilers, it is hard for developers to exploit the benefits of this new architecture. We present T10, the first DL compiler to exploit the inter-core communication bandwidth and distributed on-chip memory on AI chips. To formulate the computation and communication patterns of tensor operators in this new architecture, T10 introduces a distributed tensor abstraction rTensor. T10 maps a DNN model to execution plans with a generalized compute-shift pattern, by partitioning DNN computation into sub-operators and mapping them to cores, so that the cores can exchange data following predictable patterns. T10 makes globally optimized trade-offs between on-chip memory consumption and inter-core communication overhead, selects the best execution plan from a vast optimization space, and alleviates unnecessary inter-core communications. Our evaluation with a real inter-core connected AI chip, the Graphcore IPU, shows up to 3.3$\times$ performance improvement, and scalability support for larger models, compared to state-of-the-art DL compilers and vendor libraries.

==> backgroun_new_bak.tex <==
\section{Background and Motivation}
\label{sec:background}

\input{figures/table_compare} %TODO: remove TPU

\subsection{Distributed On-chip Memory Architecture}
%TODO: add a figure to illustrate the key difference
To meet the increasing demand for higher memory throughput in modern DNN computations, many DNN accelerators \cite{ipu2, samba, tenstorrent, wse2, h100} adopt a distributed on-chip memory architecture, where a single chip accommodates multiple parallel cores, and each core is equipped with a dedicated local memory and interconnected through a high-speed on-chip network.
Despite differences in hardware specifications, their commonality lies in two aspects: fast on-chip inter-connections across cores and large on-chip memory capacity.

This section explores the implications of such architectural changes on deep learning workloads by comparing a representative accelerator with \textit{distributed on-chip memory} — Graphcore's Intelligence Processing Unit (IPU) — with the NVIDIA A100 GPU, which is the most representative \textit{shared-memory}-based accelerator. Both share 7nm processing technology and have die areas of around 800 $mm^2$. \Cref{tab:compare_arch} lists their major hardware specifications.

\paragraph{Large distributed on-chip memory for higher bandwidth.}
Accelerators like IPUs feature large distributed on-chip memory, with each core owning a private SRAM partition as a local scratchpad memory, as illustrated in Figure~\ref{fig:xx}. As indicated in \Cref{tab:compare_arch}, the on-chip memory capacity of an IPU chip is 10$\times$ larger than that of a GPU. This enables the accommodation of large tensor operators or even an entire model within the chip. Consequently, the aggregated on-chip memory delivers significantly higher and more scalable memory throughput than off-chip memory, e.g., 8TB/s in IPU versus 1.5TB/s in GPU.
This characteristic not only enhances the efficiency of these accelerators in handling memory-intensive DNN computations, such as large language model inference~\cite{}, but also facilitates a higher computational density for scaling up the effective computation throughput in future accelerator designs.

\paragraph{Fast inter-core connection for higher scalability.}
The most notable architectural difference between IPU-like accelerators and GPUs is the high-speed inter-core connections.
This leads to a significant distinction between their data access paths.
In a GPU, each core (e.g., SM) can directly access data from a global memory with a unified address space shared among all cores.
In contrast, accelerators like IPUs typically incorporate a network-on-chip (NoC) connecting cores to enable data access from each other's local memory.
Specifically, IPUs adopt a bulk-synchronous parallel (BSP) computation model, which executes \textit{computation} and \textit{communication} phases alternately.
During the communication phase, processors synchronize and gather the required data from each other, while the computation phase involves only local data access without inter-core communication. 
Such on-chip network with distributed memory could facilitate higher parallelism, e.g., 1472 cores in IPU versus 108 in GPU, owing to its greater scalability than a centralized memory controller in GPU. 
Additionally, the inter-core communication mechanism allows data I/O to primarily occur in the on-chip network, effectively bypassing off-chip memory path with limited bandwidth and largely mitigating the off-chip memory bandwidth wall \cite{memory_wall}.
However, the distributed memory and the BSP model also introduce a greater challenge in partitioning and optimizing computations compared to the shared memory abstraction in GPUs. This motivates us to design a compiler approach to automatically handle the scheduling complexity at a transparent software layer.

\paragraph{Limitation of memory capacity.}
Despite the aforementioned advantages, a common limitation of these distributed-memory accelerators is their on-chip memory capacity, often significantly smaller than the off-chip memory in GPUs. While acknowledging this, our optimism about this architecture's potential is grounded in two key reasons.
Firstly, a distributed architecture is inherently easier to scale regarding memory capacity. This could be achieved by either scaling up local memory capacity, e.g., leveraging new memory technologies like 3D-stacking~\cite{}; or scaling out the NoC to connect more processors. For instance, the IPU mk2 chip has already tripled the memory capacity compared to IPU mk1~\cite{}. The Cerebras CS2 already boasts a 40GB on-chip memory capacity on a single chip~\cite{}.
Secondly, the large connected on-chip memory facilitates higher data reuse, effectively reducing off-chip memory I/O during the same computation. For example, an IPU can ideally accommodate an 896MB data tile in on-chip memory, significantly larger than the 20MB data tile in an A100 GPU. To compute a large matrix multiplication, this implies that an IPU could achieve $\sqrt{896MB/20MB}=6.7$ times higher operational intensity than a GPU~\cite{roofline}. Consequently, attaching a low-bandwidth off-chip memory (e.g., 1555GBps(GPU)/6.7=232GBps) is sufficient for an IPU to attain a comparable computing throughput to a GPU.
Given these promising hardware opportunities, this paper primarily focuses on software optimization exclusively in the on-chip memory of one or multiple chips.


\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/ipu-SaveSpace.drawio.pdf}
    \vspace{-3ex}
    \caption{Improve on-chip memory usage on distributed on-chip memory-based accelerators.}
    \label{fig:save_mem}
    \vspace{-2ex}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.76\linewidth]{figures/motiv_mem_duplicate.pdf}
    \vspace{-3ex}
    \caption{Data duplication ratio of various operators on IPU.}
    \label{fig:ipu_mem_duplication}
    \vspace{-2ex}
\end{figure}

\subsection{Inefficiency of Existing Approach}\label{sec:limit_existing_approach}
Given the challenge of optimizing computation on distributed memory, existing compilers~\cite{ansor,roller} or libraries~\cite{popart} for such accelerators attempt to address this by allocating a portion of local memory in each processor and abstracting them as a virtual global memory, as illustrated in \Cref{fig:save_mem}. By default, all tensors of a model are placed in the virtual global memory. During execution, similar to a shared memory accelerator, each processor retrieves the required data from the virtual global space to its remaining local memory and subsequently performs the local computation.

While such abstraction simplifies programming, it introduces significant inefficiencies. First, allocating a large portion of local memory for the virtual global memory restricts each processor to accommodate a very small sub-operator size, resulting in a notably \textit{low operational intensity} (as discussed earlier) and overall performance degradation. Second, partitioning tensors to virtual global memory could easily introduce \textit{imbalanced memory access} across processors, where one partition is accessed more frequently than others, detrimentally affecting overall performance. Third, partitioning to virtual global memory could generate many small fragmentations, causing a processor to fetch data from multiple other processors physically, leading to a \textit{high communication overhead}. Finally, fetching data from virtual global memory to local memory essentially creates data duplication in the on-chip memory space, causing \textit{significant memory space waste}. Our measurements of some typical DNN operators (\Cref{fig:ipu_mem_duplication}) show that a large operator may consume up to 5 times the on-chip memory compared to its actual variable size. This implies that more than 80\% of on-chip memory is utilized for duplicated data for individual operators, in addition to the space reserved for virtual global memory.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/ipu-motivation_example.drawio.pdf}
    \vspace{-2ex}
    \caption{Fit operator into cores with limited capacity using shift, assuming each core can hold 11 square elements.}
    \label{fig:motivation_example}
    \vspace{-2ex}
\end{figure*}

\subsection{Core Idea of \oursys{}}
% regular data access observation->rotating tensors
% duplicated tensor can be further partitioned -> 1) no memory waste -> 2) large op tile 
% equal partition -> balanced communication; 
% align computation with communication tile  -> one data transfer at a time

Given the aforementioned inefficiencies of virtual global memory approach, our goal is to explicitly partition the computation and tensors to the distributed processors and memory spaces, and organize the computation across processors as one or more pipelines, so that each processor can independently computes a partitioned task with the data received from its upstream neighbours, stores the result within itself and passes it downstream.
Such computing paradigm is a general form of systolic computation~\cite{systolic}, which is commonly used to design hardware core by organizing a group of computing units in a systolic array~\cite{tpu_v4i,eyeriss}.
The feasibility of applying such computing model for general DNN is bolstered by our observation on DNN computation patterns: most DNN operators can be divided into regular computation tasks, which load consecutive data tiles from input tensors and produce consecutive data tiles for the output tensor. 
By organizing the computation in a systolic style, every processor can compute one data tile at a time by continuously shifting the data tiles across processors.
This motivates us to design a general systolic-based approach to map and optimize the DNN computation on distributed memory-based accelerators. 

\Cref{fig:motivation_example} illustrates a simple example that maps a matrix multiplication (MatMul) operator shown in \Cref{fig:motivation_example}(a) to two cores. We first partition the operator along \textit{m} dimension into two cores as shown in \Cref{fig:motivation_example}(b), where the weight tensor needs to be used by both cores. To facilitate the above idea, we can partition the weight tensor into two consecutive columns and place it on the two cores. Then the computation can be conducted in two rounds. Each core holds half of the weight tensor and completes half of its computation per round. Between rounds, the cores shift their partitions to the next cores. After all rounds, the computation is completed.

Such computation pattern in this case perfectly avoids all the inefficiencies in virtual global memory abstraction. First, each partition of the weight tensor is stored in at least one core at any time, eliminating the need for a global memory to store shared data. This ensures maximum memory space utilization and achieves the largest possible sub-operator size. Furthermore, since we partition the tensor equally across cores, the communication volume is evenly distributed across core-to-core connections. Finally, as we can accurately align the computation task with the data tile, e.g., \Cref{fig:motivation_example}(c) shifts 2$\times$1 weight tiles and then computes a 2$\times$1 output tile, every core only needs to communicate with one other core at a time, avoiding fragmented communication with multiple cores.




% Instead of relying on global memory abstraction, our approach is to partition each operator into sub-operators, which collaboratively hold the entire tensor data across all cores, as depicted in \Cref{fig:save_mem}(c). Moreover, to prevent data duplication, the data used by a group of sub-operators can be distributed across multiple computing rounds. Consequently, one piece of data can be temporally shared among multiple sub-operators on multiple cores by shifting through the inter-core links. As a result, global memory abstraction is no longer necessary, freeing up a large portion of local memory for sub-operator execution. This method could also reduce data fetching from remote cores, as part of the data is explicitly placed in the local memory of each core.




% \textbf{Intra-operator trade-off.}
% Partitioning an operator into more cores or more computation rounds offers a trade-off between duplication and data transfer volume. For instance, slicing and shifting a small tensor over multiple rounds may save little memory space while incurring considerable synchronization overhead. On the other hand, slicing a large tensor could save significant memory with a relatively minor cost of communication. Simultaneously, the trade-off is also influenced by the local computation efficiency of different sub-operator shapes. For example, the AMP unit in IPU prefers a longer input dimension to amortize the weight-reloading overhead. \Cref{fig:shape_example} illustrates an improved partition plan compared to \Cref{fig:motivation_example}, which enables higher FLOPS by increasing the input dimension length. However, it also increases duplication by copying the 8-element output instead of the 4-element weight. This means more data must be shifted per round to eliminate duplication, resulting in higher latency. Therefore, an effective evaluation method is necessary to determine the optimal trade-off (\S\ref{sec:design:intra_op}).
% % by considering all factors .

% \vspace{0.2em}
% \noindent
% \textbf{Inter-operator trade-off.}
% \hl{Our designs are driven by a singular objective: best utilizing the on-chip memory. This is motivated by our key observation that DSM-based architecture has fundamentally changed the compiler optimization trade-off space: from optimizing data reuse to improving memory utilization.}
% Due to the limited off-chip memory bandwidth of DSM accelerators, the common practice is to place all operators in the on-chip memory to avoid off-chip memory access during computation. To further improve memory utilization, tensors in the on-chip memory are reused as much as possible. For example, weights can be reused across inference batches, and activation tensors from producer operators can be reused by consumer operators.
% \hl{If one operator uses the output tensor of the preceding operator as its input tensor, this tensor can stay in the on-chip memory to reduce expensive off-chip data transfer.}

% This pattern introduces two additional trade-off decisions.
% % First, given that different operators may have different intra-operator trade-off ratios (i.e., latency reduced by increasing the same memory capacity),  Therefore, we must globally consider the memory space allocation for each operator to maximize overall efficiency.
% First, some operators benefit more from data duplication, while some benefit less (e.g., duplicating small operators greatly reduces synchronization overhead with little memory capacity overhead). Thus, we must globally consider the trade-off between data duplication and data transfer for all operators to maximize overall efficiency.
% \hl{Therefore, instead of deliberately minimizing the data transfer overhead, we holistically optimize the end-to-end execution latency under the constraint of on-chip memory capacity.}
% Second, data duplication may be unnecessary when the operator is not executing. 
% \hl{Under this scenario, we want to reserve more memory for the currently active operator while keeping other operators in the limited on-chip memory.}
% Each operator can be stored in a memory-efficient plan (e.g., no duplication) when idle and switch to a compute-efficient plan (with duplication) during execution at the cost of a warm-up process to switch between the plans. 
% This offers a more complicated trade-off across operators among data duplication, data transfer, and warm-up (\S\ref{sec:design:inter_op}).






==> background.tex <==


\section{Background and Motivation}
\label{sec:background}

Distributed (shared) memory-based or DSM accelerators are a new branch of deep learning accelerators, offering unique features, compared to previous accelerators like GPUs and TPUs~\cite{ipu2,a100,tpu_cloud,tpu_v4i}. To highlight the differences, we compare a state-of-the-art (SOTA) DSM accelerator -- Graphcore's Intelligence Processing Unit (IPU), with Google TPU v4 and Nvidia GPU A100 in \Cref{fig:compare_arch} and \Cref{tab:compare_arch}. They share 7nm processing technology and die areas of around $800 mm^2$.

\hl{The DNN compiler for shared memory architectures like GPUs has been a prominent subject in the system community. This paper focuses on this new type of accelerator architecture, which changes the memory architecture from shared one to distributed one. We have observed that this alteration is driving a fundamental trend in AI accelerator development that facilitates higher scalability of computation \mbox{\cite{ipu2, samba, tenstorrent, wse2}}. Consequently, this change has substantially transformed the tradeoff space in DNN compiler optimization: from maximizing data reuse (better utilize off-chip memory bandwidth), to facilitating more efficient memory utilization (better utilize on-chip memory capacity). We aim to systematically explore this new space and address the associated challenges.}

% As a new branch in the family of machine learning hardware, accelerators with distributed shared memories (DSM) share several unique features against previous accelerators like Graphic Processing Units (GPU) and Tensor Processing Unit (TPU) \cite{ipu2,a100,tpu_cloud,tpu_v4i}. 
% To understand why compiling for DSM can be fundamentally different, we first compare a state-of-the-art (SOTA) DSM accelerator, the Intelligence Processing Unit (IPU) by Graphcore, to the SOTA models of other accelerator types in \Cref{fig:compare_arch} and \Cref{tab:compare_arch}. 
% As comparable peers, Google TPU v4, Nvidia GPU A100, and Graphcore IPU mk2 share the same processing technology of 7nm, similar peak performances, and similar die areas of around $800 mm^2$. 
%Meanwhile, Cerebras Wafer Scale Engine 2 (WSE2) has a giant area of $46225 mm^2$ and $50 \times$ more transistors than others \cite{wse2}.



\subsection{Large On-chip Distributed Shared Memory}
\label{sec:background:large_memory}

DSM accelerators like IPUs have large distributed on-chip memory, with each core owning a private SRAM partition as a local scratchpad (\Cref{fig:compare_arch}). Cores are directly connected, and there is no shared global on-chip memory. Such a memory hierarchy is highly scalable in both bandwidth and capacity, making it easy to increase the number of independent memory partitions. 
As shown in \Cref{tab:compare_arch}, the on-chip memory capacity of an IPU chip is 3 to 10 times larger than TPU or GPU. By fitting more data on-chip, IPU accommodates larger tensor operators and enables higher computation density with more data-reuse opportunities. This reduces off-chip memory IO when performing the same computation and largely mitigates the off-chip memory bandwidth wall \cite{memory_wall}. 

\hl{For instance, by using a data tile of size [N, N] in a matrix multiplication (MatMul) operator, the operational intensity becomes N ($N^3$ arithmetic operations divided by $N^2$ elements read). Consequently, the on-chip memory capacity plays a crucial role in determining the maximum size of a data tile that can be accommodated, as well as the required memory bandwidth for the lower-level memory layer.}
\hl{More specifically, an IPU can ideally accommodate an 896MB data tile, while an A100 GPU can ideally accommodate a 40MB data tile in its global L2 cache. For the MatMul operator, the IPU can accommodate 896MB/40MB=22 times larger tile size ($N^2$) than the GPU, so the operational intensity (N) on the IPU is sqrt(22)=4.7 times higher than on GPU. Thus, for IPU to achieve comparable compute throughput of GPU (both using off-chip memory), the off-chip memory bandwidth of IPU should be at least 1555GBps(GPU)/4.7=330.85GBps. However, the current IPU only has 32GBps off-chip memory bandwidth, which requires us to enable higher operational intensity (i.e., data reuse).}
\hl{Thus, while TPU and GPU possess smaller on-chip memory than the IPU, their off-chip memory bandwidths are sufficient to feed data even with lower data reuse. In contrast, the IPU relies on significantly larger data tiles and high data reuse to fully utilize the computation power. This motivates us to facilitate the collaborative execution of very large computation tiles across distributed memory.}

Meanwhile, the absence of global memory also prevents DSM accelerators to have a universal memory space across the chip, introducing compilation challenges. For example, while tensor variables can be simply declared and allocated into the GPU memory, they must be explicitly partitioned and assigned to local memory of specific cores on IPU \cite{ipu_hardware}. To facilitate our discussion, we will use 
IPU architecture as a representative example of DSM accelerators in this paper. 

% Implied by it name, DSM accelerators like IPU feature extremely large distributed on-chip memory, where each processing core owns one private static random-access memory (SRAM) partition as its local scratchpad, as shown in \Cref{fig:compare_arch}. 
% While each core is directly connected to other core using different topology, there is no global on-chip memory shared by all cores on DSM accelerators.
% Such on-chip memory hierarchy is highly scalable in both bandwidth and capacity, because increasing the number of independent memory partitions is convenient. 
% As shown in \Cref{tab:compare_arch}, the on-chip memory capacity on IPU is 3 or 10 times of that on TPU or GPU.
% By fitting more data into the chip, IPU accommodates larger tensor operators and enables higher computation density with more data-reuse opportunities \cite{roller}. 
% Thus, IPU transfers less data with off-chip memories to perform the same computation, and saturates its compute power without using the expensive high bandwidth memory equipped by both GPU and TPU.
% In this way, IPU mitigates the off-chip memory bandwidth wall encountered by other accelerators \cite{memory_wall}.

% However, absence of global memory prevents DSM accelerators to have a universal memory space across the entire chip, which introduces additional compilation challenges.
% For example, while tensor variables can be simply declared and allocated into the GPU memory, they must be explicitly partitioned and have each of the parts assigned to the local memory space of one specific core on IPU \cite{ipu_hardware}.



\subsection{Large Number of Small Cores}
\label{sec:background:many_small_cores}

The highly scalable IPU architecture features a larger number of smaller cores compared to other devices. IPU cores have similar functional units as TPU cores and GPU stream multiprocessors (SM), including vector processing units (VPU) or single-instruction-multiple-data (SIMD) units for element-wise computation, and matrix units (MXU), and accumulating matrix product (AMP) units for MatMul and convolution.
As shown in \Cref{tab:compare_arch}, IPU cores have the smallest SIMD width. While TPU increases MXU size to improve compute density and reduce bandwidth pressure on its large on-chip memory \cite{tpu_supercomputer}, IPU enables a smaller AMP size by leveraging the high bandwidth DSM with smaller partitions. IPU achieves comparable peak performance with TPU and GPU by increasing the number of cores. Narrower SIMD width allows tensors of various shapes to fill the SIMD array more easily, leading to higher utilization on IPUs~\cite{ipu_citadel} compared to TPUs (e.g., less than 50\%\cite{tpu_supercomputer}).

% Given its highly scalable hierarchy, IPU features a larger number of smaller cores than other devices. 
% IPU cores have similar function units with TPU cores and GPU stream multiprocessors (SM). 
% They equip vector processing units (VPU) or single-instruction-multiple-data (SIMD) units for element-wise computation.
% They also equip matrix units (MXU), TensorCores (TC), or accumulating matrix product (AMP) units to do matrix multiplication (MatMul) and convolution.



% As shown in \Cref{tab:compare_arch}, IPU cores have the smallest sizes in term of SIMD width.
% While TPU increases the MXU size to improve its compute density and reduce the pressure on the bandwidth of its large on-chip memory \cite{tpu_supercomputer}, IPU enables small AMP size by exploiting the scalable high bandwidth of its DSM with smaller size per partition.
% Meanwhile, IPU achieves comparable peak performance with TPU and GPU by increasing the number of cores.
% With narrower SIMD width, tensors of various shapes fill up the SIMD array more easily. 
% While fewer tensors are aligned to TPU's 4096-bit width, more tensors are aligned to IPU's 64-bit width.
% Thus, while the MXU spatial utilization on TPU is usually less than 50\% \cite{tpu_supercomputer}, the AMPs on IPUs have higher spatial utilization under the same workloads \cite{ipu_citadel}.

However, a large number of cores implies a large search space for partition plans, making compilation more challenging. Moreover, the systolic arrays in IPU's AMP accelerate MatMuls by preloading one input matrix as weight \cite{tpu_supercomputer, a100, ipu_isa}. If the weight is not well reused in a sub-operator, frequent weight reloading will hurt performance. Compilers must consider generating better sub-operator shape that has more data reuse to amortize the preloading cost. 

% However, since one large tensor operator need to be partitioned into small sub-operators so that each core can handle some of them, larger number of cores implies larger search space of partition plans and makes compilation more challenging.
% Further, similar to those in MXU and TC, the systolic arrays in IPU's AMP accelerate MatMuls by loading one of the input matrices as weight before actual computation \cite{tpu_supercomputer,a100,ipu_isa}. 
% If the loaded weight is not well reused in a sub-operator, frequent weight reloading may hurt the floating point operators per second (FLOPS) performance.
% Thus, an efficient compiler takes all performance factors into consideration and attempts to generate larger sub-operators.



\subsection{Inter-core Synchronization Model} 
\label{sec:background:inter_core_sync}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/ipu-bsp.drawio.pdf}
    \vspace{-2ex}
    \caption{Tensor operator runs in BSP model on IPU.}
    \label{fig:bsp}
    \vspace{-2ex}
\end{figure} 

IPUs feature small cores, resulting in reduced hardware complexity and simplified functionality, including the lack of a dedicated per-core data exchange module \cite{ipu_overlap}. In contrast, large SMs on GPUs can access data during computation from global memory, off-chip memory, or host memory. IPUs enforce a bulk-synchronous parallel (BSP) model between cores, as illustrated in \Cref{fig:bsp}, allowing inter-core communication only when no cores are computing \cite{bsp}. During the data transfer phase, cores synchronize and gather required data from other cores, while the computation phase involves only local data access without inter-core communication. This pattern ensures predictable performance due to deterministic data transfer times and no data idleness during computation.
\hl{Further, accelerators like IPU implement a network on chip that enables direct all-to-all connections between all cores. All connections have the same bandwidth, and similar latency (difference is less than 50ns\mbox{~\cite{ipu_citadel}}, while data transfers are mostly microsecond-level). Thus, physical locations of cores have negligible impact on communication overhead.}
\hl{Thus, the synchronization overhead and the communication bandwidth can be accurately measured as 118 cycles and 3.57 bytes per cycle per core, respectively, on IPU.}


% Smaller cores in IPU imply lower hardware complexity and simplified functionalities, including the absence of dedicated per-core data exchange module in IPU.
% In GPU, larger SMs access the data in global memory, off-chip memory, or even the host memory while doing computation. 
% However in IPU, each smaller core can only perform computation using the data already inside its local memory, but it cannot access data from other cores using direct links during computation.
% As shown in \Cref{fig:bsp}, IPU enforces bulk-synchronous parallel (BSP) model between its cores, where inter-core communication only happens when none of the cores are computing \cite{bsp}.
% In the data transfer phase before computation, all cores sync and gather their required data from other cores. 
% During the computation phase of each round, each cores accesses local data only and no inter-core communication happens.
% Such pattern makes performance highly predictable, since data transfer time per round is deterministic and there will be no data idleness inside computation.

Despite the advantages of reduced hardware complexity and predictable performance, the BSP model necessitates a compiler that balances the length of per-core sub-operators to prevent cores from waiting for synchronization. Additionally, an efficient compiler should minimize inter-core communication volume, as the BSP model does not overlap data transfer with computation, e.g., by increasing core-level data reuse with larger sub-operators, as suggested in \Cref{sec:background:large_memory}.

% While benefiting hardware complexity and performance prediction, BSP requires the compiler to balance the length of per-core sub-operators, so that cores do not wait for each other for sync. 
% Further, though on-chip communication on IPU is fast thanks to the lightning inter-core links, BSP does not overlap data transfer with computation. 
% Thus, an efficient compiler must also minimize the inter-core communication volume, and one solution is to increase the core-level data reuse by enabling larger sub-operators, as implied in \Cref{sec:background:large_memory}.

Meanwhile, data transfers with off-chip memory are handled transparently on IPU, but under limited bandwidth. 
A small number of cores will fetch the data from off-chip memory to their local memories when most cores are computing, then during the data transfer phase, the buffered data will be distributed to destination cores via the on-chip links \cite{ipu_overlap}.

\hl{However, as shown in \mbox{\Cref{tab:compare_arch}}, IPUs have extremely limited off-chip memory bandwidth, which is only 2\% of that on GPUs. Thus, the penalty for moving data between on-chip and off-chip memory is extremely high. To avoid stalling computation due to off-chip memory accesses, the standard way is to store all data required by the entire DNN workload in the on-chip memory prior to execution.}
\hl{When the program cannot fit into a single chip, the user can leverage multiple chips to support larger model sizes or batch sizes.
For example, in a pipeline of IPU chips, each chip handles multiple layers of the DNN model \mbox{\cite{ipu_bert_pipeline}}. Under this scenario, it is still necessary to schedule and coordinate the tensor operators running on each individual chip.}



%\subsection{DSM programming model}
%\label{sec:background:program}
%\todo{Jilong: should we remove this section?}
%The above features determine how tensor operators are executed on DSM hardware like IPU, as shown in \Cref{fig:bsp}.
%First, each partition of the tensor variables must be allocated to a specific core.
%Also, each arithmetic operator on tensors must be partitioned into several rounds of sub-operators for each core. 
%For each round, each core gathers required data from peers using the inter-core links and then execute one sub-operator using local data.
%After the round, cores synchronize with each other and start the next round.

==> background_new_bak2.tex <==
\section{Background and Motivation}
\label{sec:background}

\input{figures/table_compare} %TODO: remove TPU

% \subsection{Distributed On-chip Memory Architecture}
\subsection{Massively Parallel Intelligence Processor}
%TODO: add a figure to illustrate the key difference
To meet the increasing demand for higher memory throughput in modern DNN computations, many DNN accelerators \cite{ipu2, samba, tenstorrent, wse2, h100} adopt a distributed on-chip memory architecture, where a single chip accommodates multiple parallel cores, and each core is equipped with a dedicated local memory and interconnected through a high-speed on-chip network.
Despite differences in hardware specifications, their commonality lies in two aspects: fast on-chip interconnections across cores and large on-chip memory capacity.

This section explores the implications of such architectural changes on deep learning workloads by comparing a representative accelerator with \textit{distributed on-chip memory} — Graphcore's Intelligence Processing Unit (IPU) — with the NVIDIA A100 GPU, which is the most representative \textit{shared-memory}-based accelerator. Both share 7nm processing technology and have die areas of around 800 $mm^2$. \Cref{tab:compare_arch} lists their major hardware specifications.

% core-to-core bandwidth 6GB/s
% all-to-all bandwidth 8TB/s
% aggregated SRAM BW (during compute phase) 45TB/s
\noindent
\textbf{High-speed inter-core connection.}
The most notable architectural difference between IPU-like accelerators and GPUs is the high-speed inter-core connections.
This leads to a significant distinction between their data access paths.
On a GPU, each core (e.g., SM) can directly access data from a global memory with a unified address space shared among all cores.
In contrast, an IPU incorporates a network-on-chip (NoC) connecting cores to enable data access from each other's local memory.
To ease the programming effort of managing inter-core synchronizations, IPUs adopt a bulk-synchronous parallel (BSP) computation model, which executes \textit{computation} and \textit{communication} phases alternately.
During the communication phase, all cores synchronize and gather the required data from each other, while the computation phase involves only local memory access without inter-core communication.

Thanks to the high-speed on-chip network, a distributed on-chip memory can scale to a much higher aggregated bandwidth than the shared-memory architecture.
On a GPU, all cores fetch data from the on-chip L2 cache, which can only provide limited bandwidth (about 5TB/s on A100~\cite{gpu_bandwidth}).
In addition, when different cores access different data, the actual bandwidth will be much lower due to contentions.
On an IPU, the peak inter-core all-to-all bandwidth (i.e., the aggregated bandwidth for all cores to fetch data from other cores) is much higher (about 8TB/s~\cite{ipu_hardware}),
which makes IPU-like accelerators an ideal fit for memory bandwidth-intensive DNN workloads.
% First, it facilitates higher parallelism, e.g., 1472 cores in IPU versus 108 in GPU, owing to its greater scalability than a centralized memory controller in GPU.
% Additionally, the inter-core communication mechanism allows data I/O to primarily occur in the on-chip network, effectively bypassing off-chip memory path with limited bandwidth and largely mitigating the off-chip memory bandwidth wall \cite{memory_wall}.
However, to fully exploit the on-chip network bandwidth, the software must carefully manage the data placement and schedule inter-core communications to avoid unnecessary data access conflicts and redundant data fetches. This poses a significant challenge for the DNN compiler design.
% partition and optimize computations compared to the shared memory abstraction in GPUs. This motivates us to design a compiler approach to automatically handle the scheduling complexity at a transparent software layer.

\noindent
\textbf{Large distributed on-chip memory.}
Accelerators like IPUs often feature much larger on-chip memory than GPUs. As indicated in \Cref{tab:compare_arch}, the on-chip memory of an IPU chip is 10$\times$ larger than that of a GPU.
This is because the inter-core connections enable all cores to access each other's local memory, so they do not need to rely on a global on-chip memory (like the L2 cache on a GPU) to synchronize data.
Therefore, the saved hardware budget from removing the global cache can be spent on adding more cores and enlarging each core's local memory, resulting in a much larger aggregated on-chip memory capacity.
As a result, the larger on-chip memory can accommodate a larger tile size for tensor operators or even an entire model within the chip. This characteristic not only enhances the efficiency of these accelerators in handling memory-intensive DNN computations, such as large language model inference~\cite{llm_inference_characteristics}, but also facilitates a higher computational density for scaling up the effective computation throughput in future accelerator designs.

% The large on-chip memory of IPUs enables the accommodation of large tensor operators or even an entire model within the chip.
% Consequently, the aggregated on-chip memory delivers significantly higher and more scalable memory throughput than off-chip memory, e.g., 8TB/s in IPU versus 1.5TB/s in GPU.


% \paragraph{Limitation of memory capacity.}
\noindent
\textbf{Limitations of the current IPU hardware.}
In this paper, we prototype \oursys{} with IPUs, as we currently do not have access to other distributed on-chip memory-based accelerators. As a recently developed accelerator, the current IPU still exhibits some limitations. These limitations are not fundamental to the distributed on-chip memory architecture, and we anticipate that future generations of IPUs will address them.

First, an IPU chip is not equipped with high-bandwidth off-chip memory, such as the HBM on GPUs~\cite{ipu2}. Instead, it is designed to fit the entire DNN model into the 900MB on-chip memory to exploit the high SRAM bandwidth.
To support larger models, multiple IPU chips can be connected to scale out the memory capacity.
% While the 900MB memory per chip is sufficient for most models except LLMs, the limited capacity still brings significant challenges for compiler optimizations.
To this end, our \oursys{} implementation mainly targets an IPU chip without off-chip memory, but it can be easily extended to support a hypothetical IPU chip with HBM (see our discussion in~$\S$\ref{sec:discussion}).

Second, the computation phase and communication phase cannot overlap on an IPU chip since there is no independent network-on-chip controller in each core.
While this design choice relieves programming efforts and simplifies hardware design, it causes sub-optimal performance.
We anticipate that future generations of IPUs may support this feature.

% Despite the aforementioned advantages, a common limitation of these distributed-memory accelerators is their on-chip memory capacity, often significantly smaller than the off-chip memory in GPUs. While acknowledging this, our optimism about this architecture's potential is grounded in two key reasons.
% Firstly, a distributed architecture is inherently easier to scale regarding memory capacity. This could be achieved by either scaling up local memory capacity, e.g., leveraging new memory technologies like 3D-stacking~\cite{}; or scaling out the NoC to connect more processors. For instance, the IPU mk2 chip has already tripled the memory capacity compared to IPU mk1~\cite{}. The Cerebras CS2 already boasts a 40GB on-chip memory capacity on a single chip~\cite{}.
% Secondly, the large connected on-chip memory facilitates higher data reuse, effectively reducing off-chip memory I/O during the same computation. For example, an IPU can ideally accommodate an 896MB data tile in on-chip memory, significantly larger than the 20MB data tile in an A100 GPU. To compute a large matrix multiplication, this implies that an IPU could achieve $\sqrt{896MB/20MB}=6.7$ times higher operational intensity than a GPU~\cite{roofline}. Consequently, attaching a low-bandwidth off-chip memory (e.g., 1555GBps(GPU)/6.7=232GBps) is sufficient for an IPU to attain a comparable computing throughput to a GPU.
% Given these promising hardware opportunities, this paper primarily focuses on software optimization exclusively in the on-chip memory of one or multiple chips.


\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/ipu-SaveSpace.drawio.pdf}
    \vspace{-3ex}
    \caption{Improve on-chip memory usage on distributed on-chip memory-based accelerators.}
    \label{fig:save_mem}
    \vspace{-2ex}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.76\linewidth]{figures/motiv_mem_duplicate.pdf}
    \vspace{-3ex}
    \caption{Data duplication ratio of various operators on IPU.}
    \label{fig:ipu_mem_duplication}
    \vspace{-2ex}
\end{figure}

\subsection{Inefficiency of Existing Approach}\label{sec:limit_existing_approach}
Given the challenge of optimizing computation on distributed memory, existing compilers~\cite{ansor,roller} or libraries~\cite{popart} for such accelerators attempt to address this by allocating a portion of local memory in each processor and abstracting them as a virtual global memory, as illustrated in \Cref{fig:save_mem}. By default, all tensors of a model are placed in the virtual global memory. During execution, similar to a shared memory accelerator, each processor retrieves the required data from the virtual global space to its remaining local memory and subsequently performs the local computation.

While such abstraction simplifies programming, it introduces significant inefficiencies. First, allocating a large portion of local memory for the virtual global memory restricts each processor to accommodate a very small sub-operator size, resulting in a notably \textit{low operational intensity} (as discussed earlier) and overall performance degradation. Second, partitioning tensors to virtual global memory could easily introduce \textit{imbalanced memory access} across processors, where one partition is accessed more frequently than others, detrimentally affecting overall performance. Third, partitioning to virtual global memory could generate many small fragmentations, causing a processor to fetch data from multiple other processors physically, leading to a \textit{high communication overhead}. Finally, fetching data from virtual global memory to local memory essentially creates data duplication in the on-chip memory space, causing \textit{significant memory space waste}. Our measurements of some typical DNN operators (\Cref{fig:ipu_mem_duplication}) show that a large operator may consume up to 5 times the on-chip memory compared to its actual variable size. This implies that more than 80\% of on-chip memory is utilized for duplicated data for individual operators, in addition to the space reserved for virtual global memory.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/ipu-motivation_example.drawio.pdf}
    \vspace{-2ex}
    \caption{Fit operator into cores with limited capacity using shift, assuming each core can hold 11 square elements.}
    \label{fig:motivation_example}
    \vspace{-2ex}
\end{figure*}

\subsection{Core Idea of \oursys{}}
% regular data access observation->rotating tensors
% duplicated tensor can be further partitioned -> 1) no memory waste -> 2) large op tile 
% equal partition -> balanced communication; 
% align computation with communication tile  -> one data transfer at a time

Given the aforementioned inefficiencies of virtual global memory approach, our goal is to explicitly partition the computation and tensors to the distributed processors and memory spaces, and organize the computation across processors as one or more pipelines, so that each processor can independently computes a partitioned task with the data received from its upstream neighbours, stores the result within itself and passes it downstream.
Such computing paradigm is a general form of systolic computation~\cite{systolic}, which is commonly used to design hardware core by organizing a group of computing units in a systolic array~\cite{tpu_v4i,eyeriss}.
The feasibility of applying such computing model for general DNN is bolstered by our observation on DNN computation patterns: most DNN operators can be divided into regular computation tasks, which load consecutive data tiles from input tensors and produce consecutive data tiles for the output tensor. 
By organizing the computation in a systolic style, every processor can compute one data tile at a time by continuously shifting the data tiles across processors.
This motivates us to design a general systolic-based approach to map and optimize the DNN computation on distributed memory-based accelerators. 

\Cref{fig:motivation_example} illustrates a simple example that maps a matrix multiplication (MatMul) operator shown in \Cref{fig:motivation_example}(a) to two cores. We first partition the operator along \textit{m} dimension into two cores as shown in \Cref{fig:motivation_example}(b), where the weight tensor needs to be used by both cores. To facilitate the above idea, we can partition the weight tensor into two consecutive columns and place it on the two cores. Then the computation can be conducted in two rounds. Each core holds half of the weight tensor and completes half of its computation per round. Between rounds, the cores shift their partitions to the next cores. After all rounds, the computation is completed.

Such computation pattern in this case perfectly avoids all the inefficiencies in virtual global memory abstraction. First, each partition of the weight tensor is stored in at least one core at any time, eliminating the need for a global memory to store shared data. This ensures maximum memory space utilization and achieves the largest possible sub-operator size. Furthermore, since we partition the tensor equally across cores, the communication volume is evenly distributed across core-to-core connections. Finally, as we can accurately align the computation task with the data tile, e.g., \Cref{fig:motivation_example}(c) shifts 2$\times$1 weight tiles and then computes a 2$\times$1 output tile, every core only needs to communicate with one other core at a time, avoiding fragmented communication with multiple cores.




% Instead of relying on global memory abstraction, our approach is to partition each operator into sub-operators, which collaboratively hold the entire tensor data across all cores, as depicted in \Cref{fig:save_mem}(c). Moreover, to prevent data duplication, the data used by a group of sub-operators can be distributed across multiple computing rounds. Consequently, one piece of data can be temporally shared among multiple sub-operators on multiple cores by shifting through the inter-core links. As a result, global memory abstraction is no longer necessary, freeing up a large portion of local memory for sub-operator execution. This method could also reduce data fetching from remote cores, as part of the data is explicitly placed in the local memory of each core.




% \textbf{Intra-operator trade-off.}
% Partitioning an operator into more cores or more computation rounds offers a trade-off between duplication and data transfer volume. For instance, slicing and shifting a small tensor over multiple rounds may save little memory space while incurring considerable synchronization overhead. On the other hand, slicing a large tensor could save significant memory with a relatively minor cost of communication. Simultaneously, the trade-off is also influenced by the local computation efficiency of different sub-operator shapes. For example, the AMP unit in IPU prefers a longer input dimension to amortize the weight-reloading overhead. \Cref{fig:shape_example} illustrates an improved partition plan compared to \Cref{fig:motivation_example}, which enables higher FLOPS by increasing the input dimension length. However, it also increases duplication by copying the 8-element output instead of the 4-element weight. This means more data must be shifted per round to eliminate duplication, resulting in higher latency. Therefore, an effective evaluation method is necessary to determine the optimal trade-off (\S\ref{sec:design:intra_op}).
% % by considering all factors .

% \vspace{0.2em}
% \noindent
% \textbf{Inter-operator trade-off.}
% \hl{Our designs are driven by a singular objective: best utilizing the on-chip memory. This is motivated by our key observation that DSM-based architecture has fundamentally changed the compiler optimization trade-off space: from optimizing data reuse to improving memory utilization.}
% Due to the limited off-chip memory bandwidth of DSM accelerators, the common practice is to place all operators in the on-chip memory to avoid off-chip memory access during computation. To further improve memory utilization, tensors in the on-chip memory are reused as much as possible. For example, weights can be reused across inference batches, and activation tensors from producer operators can be reused by consumer operators.
% \hl{If one operator uses the output tensor of the preceding operator as its input tensor, this tensor can stay in the on-chip memory to reduce expensive off-chip data transfer.}

% This pattern introduces two additional trade-off decisions.
% % First, given that different operators may have different intra-operator trade-off ratios (i.e., latency reduced by increasing the same memory capacity),  Therefore, we must globally consider the memory space allocation for each operator to maximize overall efficiency.
% First, some operators benefit more from data duplication, while some benefit less (e.g., duplicating small operators greatly reduces synchronization overhead with little memory capacity overhead). Thus, we must globally consider the trade-off between data duplication and data transfer for all operators to maximize overall efficiency.
% \hl{Therefore, instead of deliberately minimizing the data transfer overhead, we holistically optimize the end-to-end execution latency under the constraint of on-chip memory capacity.}
% Second, data duplication may be unnecessary when the operator is not executing. 
% \hl{Under this scenario, we want to reserve more memory for the currently active operator while keeping other operators in the limited on-chip memory.}
% Each operator can be stored in a memory-efficient plan (e.g., no duplication) when idle and switch to a compute-efficient plan (with duplication) during execution at the cost of a warm-up process to switch between the plans. 
% This offers a more complicated trade-off across operators among data duplication, data transfer, and warm-up (\S\ref{sec:design:inter_op}).






==> design.tex <==


% \vspace{-0.5em}
\section{System Design of \oursys{}}
\label{sec:design}
% \vspace{-0.5em}

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.62]{figures/ipu-overview.drawio.pdf}
    \vspace{-3ex}
    \caption{System overview of \pname{}.}
    \label{fig:overview}
    \vspace{-3ex}
\end{figure}



%To generalize the above idea for various DNN models and accelerators, 
We now introduce \oursys{}, a compiler designed to optimize end-to-end DNN model execution on an inter-core connected intelligence processor.
We present the overview of \pname{} in \Cref{fig:overview}: 
\textbf{(1)} \pname{} introduces the RotatingTensor (\rtensor{}) abstraction to represent the partitioning and communication patterns of tensor operators on distributed on-chip memory ($\S$\ref{sec:design:rtensor}).
\textbf{(2)} It uses the \rtensor{} to map a complete DNN model to compute-shift execution plans ($\S$\ref{sec:design:compute}).
\textbf{(3)} By configuring \rtensor{}s in different ways, \pname{} defines a comprehensive spatial-temporal optimization space for a DNN model. 
It adopts a two-staged optimization strategy to
handle the tradeoff between inter-core communication and memory footprint, and
optimize for end-to-end DNN model execution.
For each operator, \pname{} finds the Pareto-optimal execution plans that represent the best trade-off between the execution time and memory footprint ($\S$\ref{subsubsec:intra-operator}).
Then, \pname{} employs a holistic inter-operator memory reconciliation policy to determine the best 
end-to-end plan for the DNN model ($\S$\ref{subsubsec:inter-operator}).
\textbf{(4)} The generated end-to-end plan is compiled onto the processor using three abstracted device interfaces ($\S$\ref{sec:design:hardware}).
% Together, \pname{} enables efficient DNN model execution on DSM-based accelerators by optimizing both intra- and inter-operator scheduling.
% distributed memory-based accelerators.







% [TODO: introduce overview \Cref{fig:overview}]
% By incorporating the above ideas, we introduce \pname{}, a compiler designed to optimize end-to-end DNN model execution on DSM-based accelerators. The workflow of \pname{} is illustrated in \Cref{fig:overview} and consists of the following steps:




\subsection{\rtensor{}: A New Tensor Abstraction}
\label{sec:design:rtensor}


% \todo{intercore connect for general CPU is an old thing, dataflow arch is intrinsically hard to optimize (2.2), not new compute model, highlight constraints and tradeoff, use 4.3}


To map a tensor onto the distributed on-chip memory and stream the partitioned sub-tensors across multiple groups of cores, \oursys{} introduces a distributed tensor abstraction called RotatingTensor (\rtensor{}), as shown in \Cref{fig:rtensor}.
% with three new fields: a \textit{spatial partition factor} $f_s$, a \textit{temporal partition factor} $f_t$, and a \textit{rotating pace} $rp$, as shown in \Cref{fig:rtensor}.
% In addition to defining the tensor shape and data type like a normal tensor, an \rtensor{} also specifies how it is mapped and optionally rotated across a group of cores.
% All factors are vectors with a length equal to the number of dimensions of this tensor.
In addition to defining the tensor shape and data type like a normal tensor, \rtensor{} also describes how each tensor is partitioned, mapped, and shifted on the interconnected cores.

% \pname{} uses a \textit{tensor expression} of an operator \mbox{(\S\ref{sec:design:compute})} to derive its \rtensor{}s.
First, \pname{} partitions the computation of an operator onto multiple cores.
Based on the data dependency, the computation partitioning will imply how each of its input/output tensor is partitioned.
This gives a \textit{spatial partition factor} ($\bm{f_s}$), which splits a tensor into sub-tensors.
Second, each sub-tensor may be required by multiple cores.
To share a sub-tensor among them, we specify how the sub-tensor is further partitioned among the cores using a \textit{temporal partition factor} ($\bm{f_t}$).
Third, we specify how the partitions of a sub-tensor are circularly shifted among the cores using the \textit{rotating pace} ($\bmrp$).
Altogether, a set of \rtensor{}s of an operator defines a compute-shift execution plan. Given numerous possible \rtensor{} configurations of an operator, T10 forms a combinatorial optimization space of execution plans.

Specifically, $f_s$, $f_t$, and $\rp$ are vectors with a length equal to the number of dimensions of a tensor, which indicate how the tensor is partitioned along each dimension.
For example, in \mbox{\Cref{fig:shift} (a)}, a tensor $T$ of shape $[6, 8]$ is partitioned by a spatial factor $[2, 1]$, forming 2 sub-tensors of shape $[3, 8]$ along the first dimension.
Then, to share each sub-tensor among 4 cores without incurring high memory footprint, a temporal factor $f_t=[1,x]$ further partitions each sub-tensor into $x$ partitions with shape $[3, \frac{8}{x}]$, as shown in \mbox{\Cref{fig:shift} (b) and (c)}.
It forms $\frac{4}{x}$ rotation rings with $x$ cores in each, where cores share the sub-tensor by circularly shifting its partitions.
% The difference between $f_s$ and $f_t$ is that the spatially partitioned sub-tensors will be statically placed in each core's local memory, while each set of temporally partitioned sub-tensors will form a rotating ring across the intelligence cores to continuously shift tensor data to adjacent cores.
% The difference between $f_s$ and $f_t$ is that the spatially partitioned sub-tensors will be statically placed in each core's local memory,
% while each set of temporally partitioned sub-tensors will form a rotating ring across the intelligence cores to continuously shift tensor data to adjacent cores.

Finally, the rotating pace $\rp$ controls how fast an \rtensor{} is rotating, so that we can align the data shifting with computation (see \S\ref{sec:design:compute}).
Practically, $\rp$ specifies the number of data elements shifted in each step along each tensor dimension. For example, $\rp=[0, 2]$ in \Cref{fig:shift} (c) means that for each step, the sub-tensor shifts 2 elements along the second dimension (i.e., a data tile of shape $[3, 2]$), and finishes a full cycle in 4 steps.
Notably, different $\rp$s can be applied to a same set of $f_s$ and $f_t$. For instance, in \Cref{fig:shift} (d), $\rp=[0, 1]$ shifts a tile of $[3, 1]$ for each step, requiring 8 steps in total.

% \begin{figure} [t]
% \small
% \centering
% \noindent
% \begin{minipage}[t]{0.9\linewidth}
% \begin{lstlisting}
% class RotatingTensor {
%   vector<size_t> shape;
%   DataType type;
%   vector<size_t> spatial_factor;
%   vector<size_t> temporal_factor;
%   vector<size_t> rotating_pace;
% };
% \end{lstlisting}
% \end{minipage}
% \vspace{-3ex}
% \caption{\rtensor{} abstraction in \oursys{}.} 
% \vspace{-2ex}
% \label{fig:rtensor}
% \end{figure}



\begin{figure}[t]
    \centering
   % \vspace{-0.5ex}
    \includegraphics[scale=0.65]{figures/ipu-rtensor.drawio.pdf}
    \vspace{-3.5ex}
    \caption{\rtensor{} abstraction in \oursys{}.}
    \label{fig:rtensor}
    \vspace{-4ex}
\end{figure}

\begin{figure*}[t]
    \centering
    % \vspace{-0.5ex}
    \includegraphics[width=1\linewidth]{figures/ipu-rotate_new.drawio.pdf}
    \vspace{-6ex}
    \caption{Illustration of \rtensor{} partitioning and rotating.}
    \label{fig:shift}
    \vspace{-3ex}
\end{figure*}



% \vspace{-2ex}
\subsection{\textit{Compute-Shift} Execution Plan}
\label{sec:design:compute}
% \vspace{-0.3em}

Using the \rtensor{} abstraction, \oursys{} organizes the computation of a general DNN operator into a compute-shift pattern, where the operator's computation and tensors are partitioned to individual cores and their local memories.
For each step, each core computes a local \textit{sub-task}, and shifts the local tensors to its neighbors.
The entire process involves multiple compute-shift steps until each tensor has been shifted across all cores that require it.
We now discuss how \oursys{} partitions DNN operators into compute-shift-based execution plans.

\begin{figure*}[t]
    \centering
    % \vspace{-1.5ex}
    \includegraphics[scale=0.60]{figures/ipu-cannon_factor.drawio.pdf}
    \vspace{-3ex}
    \caption{An example of the rotation of \rtensor{}. The compute-shift executions of the sub-operators need to be aligned.}
    \label{fig:cannon}
    \vspace{-3ex}
\end{figure*}


\vspace{0.2em}
\noindent
\textbf{Operator representation.}
To represent an operator's computation, \oursys{} uses tensor expression~\cite{tvm, ansor, roller}, which defines how each output tensor element is computed using the input tensor values. For instance, a matrix multiplication of tensors $A$ in shape $[M, K]$ and $B$ in $[K, N]$ into $C$ is expressed as
% \oursys{} uses tensor expression~\cite{tvm, ansor, roller} to represent an operator's computation. A tensor expression defines how each output tensor element is computed based on the input tensor values. For instance, a matrix multiplication of tensors $A$ in shape $[M, K]$ and $B$ in $[K, N]$ into $C$ can be expressed as
\vspace{-0.3em}
\begin{equation}\label{eqn:matmul_texpr}
    C[m, n] \mathrel{+}= A[m, k] * B[k, n],
    \vspace{-0.3em}
\end{equation}
where $m$, $n$, and $k$ are axes to index the elements in each tensor. \Cref{eqn:matmul_texpr} indicates that any value in $C$ indexed by $m$ and $n$ (i.e., $C[m, n]$) is computed by summing $A[m, k]*B[k, n]$ over all possible indices $k$.
\oursys{} supports all common operators like MatMul and Convolution. For a few special cases like Sort, which cannot be represented in tensor expression,
\oursys{} uses the implementations from the vendor library.
% \oursys{} relies on the vendor library to provide their kernel implementations. 

\vspace{0.2em}
\noindent
\textbf{Partitioning an operator.}
To map an operator to the inter-connected cores, \oursys{} first partitions it into parallel \textit{sub-operators} along all unique axes in its corresponding tensor expression, using an \textit{operator partition factor} ($\bm{F_{op}}$).
% For example, the operator in~\Cref{eqn:matmul_texpr} can be partitioned along the $m$, $n$, and $k$ axes. We use a vector $F_{op}$ to indicate the partition factor for each corresponding axis of this operator. 
For example, \Cref{eqn:matmul_texpr} contains axes $m$, $n$, and $k$, then $F_{op}$ is a vector of three integer factors specifying how the three axes are spatially partitioned.
The total number of sub-operators is the product of all $F_{op}$ factors, so a $F_{op} = [2, 3, 1]$ for $[m,n,k]$ will slice the operator into 6 sub-operators on 6 cores, each computing a $[{\frac{M}{2}}, K] \times [K, \frac{N}{3}]$ sub-matrix multiplication.

\vspace{0.2em}
\noindent
\textbf{Partitioning \rtensor{}s.}
% Based on the operator partitioning, we can determine the partitioning for all related tensors and transform them into \rtensor{}s.
\oursys{} then uses $F_{op}$ to derive the spatial partition factor $f_s$ for each tensor, following the data dependencies in tensor expression. 
% First, \oursys{} uses $F_{op}$ to derive the spatial partition factor $f_s$ for each tensor by analyzing the data dependencies in the tensor expression. 
% For example, the above $F_{op}=[3, 2, 1]$ implies the spatial factors $[3, 1]$, $[1, 2]$, and $[3, 2]$ for tensors A, B, and C. They are split into sub-tensors of shapes $[{M\over3}, K]$, $[K, {N\over2}]$, and $[{M\over3}, {N\over2}]$.
With the same example, for $F_{op} = [2, 3, 1]$ on $[m, n, k]$, the spatial partition factor for the tensor A is $f_s^A = [2, 1]$ for axes $m$ and $k$. Similarly, for tensors B and C, we have $f_s^B = [1, 3]$ and $f_s^C = [2, 3]$.
% If a tensor dimension is a combination of multiple axes, e.g., the third dimension of tensor $I$ in~\Cref{eqn:conv_texpr} is $h+k$, \oursys{} will partition 
% along this dimension to ensure each sub-operator has all the required data.
%with an overlapped region to ensure each sub-operator has all the required data. %, which is also achieved through expression analysis.



If a tensor's dimensions do not include some axis in $F_{op}$, the partitioned sub-tensors are required by multiple sub-operators along the missing axis.
Thus, once the spatial factor determines the number of cores that will share a sub-tensor, the temporal factor determines how we split the sub-tensor across these cores into rotation ring(s).
In the above example, $F_{op}$ partitions the entire operator onto $3\times 2\times 1=6$ cores, and the spatial factor $f_s^B$ partitions tensor B into $1\times 2=2$ sub-tensors.
Thus, each sub-tensor is executed by $P=\frac{6}{2}=3$ cores.
A temporal factor $f_t^B=[3, 1]$ can further partition each sub-tensor into $3\times 1 = 3$ parts, forming $\frac{P}{3}=1$ rotation ring.
\pname{} enforces the product of factors in $f_t$ is a divisor of $P$ such that the number of rotation rings is an integer.

% For example, in Figure~\ref{fig:motivation_example} (b), the operator is partitioned by $F_{op} = [2, 1, 1]$ and the weight tensor (does not contain axis $m$) is required by both cores.
% \oursys{} can specify the temporal partition factor $f_t$ for this \rtensor{} and a rotating pace $rp$ to store and rotate these sub-tensors. 
% For example, by specifying $f_t=[1, 2]$ and $rp=[0, 1]$ for the weight \rtensor{}, we can map it to the two cores and rotate the sub-tensors for two rounds as shown in Figure~\ref{fig:motivation_example} (c).
% Note that, if a reduction dimension is partitioned, each processor will hold a partial result of the output tensor, which requires an additional reduction stage to obtain the full result.



\vspace{0.2em}
\noindent
\textbf{Aligning the rotations of \rtensor{}s.}
Since a general DNN operator can have various tensor shapes, a naive partitioning plan can easily cause the tensor shifting and the sub-task computing at an unaligned pace.
In \mbox{Figure~\ref{fig:cannon}} (a), we still use the MatMul operator in \mbox{\Cref{eqn:matmul_texpr}} as an example.
We partition it into a $2\times3$ grid in \mbox{Figure~\ref{fig:cannon}} (b), with the specified partition factors. Note that both A and B are temporally partitioned along axis $k$, but with different $f_t$ factors.

 The rotating paces of tensors in one operator need to be aligned to ensure correct data dependency.
 In \mbox{Figure~\ref{fig:cannon}} (c), tensors A and B are shifted with different $\rp$s along axis $k$, which breaks data dependency.
 In the bottom-right core, we cannot compute $C \mathrel{+}= A_2 * B_2$, as $B_2$ is not on this core after an unaligned rotation.
% By default, tensor A will be shifted in 2 steps and tensor B in 1 step, so sub-task is unable to access all its required data timely (Figure~\ref{fig:cannon} (c)).
% To organize computation into an aligned compute-shift plan,
To organize the computation into an aligned compute-shift plan, \oursys{} synchronizes the $\rp$ of each \rtensor{} (Figure~\ref{fig:cannon} (d)),
by enforcing the following constraints.

First, if a set of \rtensor{}s $\{1,2,\dots,i\}$ are rotating along the same axis (e.g., $k$), they must share the same rotating pace $\rp$ along $k$.
Let $K$ be the number of elements along $k$, and let $f_t^i$ be the temporal partition factor of \rtensor{} $i$ along $k$.
The $\rp$ values on axis $k$ must satisfy the condition
 \vspace{-0.3em}
\begin{equation}\label{eqn:rp_constraint}
    rp \leq \frac{K}{2f_t^{i}}+\frac{1}{2} \textbf{ } \textbf{ or } \textbf{ } rp=\frac{K}{f_{t}^{i}}
     \vspace{-0.3em}
\end{equation}
for all these \rtensor{}s.
% Here, $f_{t}^{i}$ represents the temporal factor of the $i$th \rtensor{} along the dimension corresponding to axis $k$, and $K$ is the length of axis $k$.
The intuition is that if the original $K/f_t^i$-sized partitions of some \rtensor{}s are unaligned (i.e., there exist two \rtensor{}s $i$ and $j$ such that $K/f_t^i \neq K/f_t^j$), we want to find an appropriate $\rp$ to reorganize each \rtensor{} into $\rp$-sized partitions and maintain the data dependency.
\hl{We elaborate on how we derive \mbox{\Cref{eqn:rp_constraint} in \Cref{appendix:rp_constraint}}.}
% The upper bound of $\rp$ ensures that, following each rotation, each new sub-tensor contains a complete new partition with a size of $\rp$ along dimension $k$.

Second, the temporal factor of each \rtensor{} should be a divisor of the number of sub-operators ($P$) that require this tensor. If $f_t^i$ is less than $P$, it is necessary to replicate each sub-tensor $P/f_t^i$ times to ensure that each sub-operator can access one partition at any given time. Although this duplication consumes memory space, it reduces the communication steps of the rotating loop, which provides a trade-off space between memory consumption and communication cost.

After satisfying the alignment constraints, we can always organize an operator's computation into a compute-shift execution plan. Specifically, in each step, each sub-operator computes a sub-task that is partitioned by the factors in $F_{op}$ and the rotating pace $\rp$ along each axis. Each sub-operator iterates over all its sub-tasks by nested-looping through the axes of this operator.
Between sub-tasks, an \rtensor{} is rotated along the currently iterating axis for all its sub-tensors. The process continues until all sub-tasks are enumerated.
% When the computation is finished, all the \rtensor{}s complete a full rotation loop.
% Figure~\ref{fig:cannon} (d) illustrates an aligned MatMul operator execution plan on a $2\times3$ cores, which is partitioned by $F_{op}=[2, 3, 1]$. The corresponding \rtensor{}s are partitioned by A=\{$f_s:[2,1], f_t:[1, 3], rp:[0, K/3]$\}, B=\{$f_s:[1,3], f_t:[2, 1], rp:[K/3, 0]$\}, C=\{$f_s:[2,3], f_t:[1, 1], rp:[0, 0]$\}.


% \vspace{-3ex}
\subsection{Intra- and Inter-operator Trade-off}
\label{sec:design:optimization}
% \vspace{-0.3em}
% \paragraph{Intra- and inter-operator optimization space.}

For each operator, there could be a vast number of execution plans involving different spatial and temporal partition factors and rotating paces. 
%Each configuration may have different impacts on computing performance, communication cost, and memory footprint. 
Moreover, an end-to-end model consists of numerous operators, creating a substantial combinatorial optimization space.
% An unoptimized execution plan not only introduces significant overhead in computation and communication, but also wastes precious memory space.
% limiting the ability to fit larger models into the processor chip. 
% For each operator, there could be a vast number of potential execution plans involving different spatial or temporal partitioning factors, rotating speeds, and others. Each configuration may have different impacts on computing performance, communication cost, and memory footprint. Moreover, an end-to-end model consists of numerous operators, creating a substantial combinatorial optimization space.
% An unoptimized execution plan not only introduces significant overhead in computation and communication, but also wastes precious memory space, 
% limiting the ability to fit larger models into an intelligence processor. 
% To optimize the execution time with the best memory space utilization, 
\oursys{} defines a \textit{two-level trade-off space between execution time and memory consumption}.

First, when determining each operator's execution plan, we can trade memory space for execution efficiency by specifying a smaller temporal partitioning factor.
This can reduce communication costs by reducing the hops in the rotation loop, while at the cost of using more memory to hold duplicated tensors.
We refer to this as \textbf{\textit{intra-operator trade-off}}.

Second, we can trade off between memory space and execution time across all operators holistically when deciding the end-to-end model execution plan.
Different operators have different memory-latency trade-offs, allowing us to allocate more memory to operators with higher memory-cost efficiency.
Moreover, a single operator can have multiple execution plans, such as utilizing a memory-efficient plan when the operator is not executing to save more memory space, and switching to an execution-efficient plan when it is about to execute.
We refer to this as \textbf{\textit{inter-operator trade-off}}.

To optimize such two-level trade-offs, \oursys{} decouples the combinatorial space into two distinct stages.
First, \oursys{} optimizes each individual operator's execution by searching for all Pareto-optimal trade-off plans between execution time and memory consumption ($\S$\ref{subsubsec:intra-operator}).
Second, \oursys{} globally optimizes the memory allocation among different operators based on the intra-operator Pareto-optimal plans ($\S$\ref{subsubsec:inter-operator}).



% \noindent
\subsubsection{Searching Pareto-optimal Intra-operator Plans}
\label{subsubsec:intra-operator}
% \vspace{-0.5em}

For each operator, to search for the optimal execution plan among numerous configuration choices, an efficient performance feedback for each plan is essential. \oursys{} leverages the unique advantage of distributed on-chip memory architecture, which involves only local computation and communication, to design a sufficiently accurate cost model.

First, given the partitioning factors of an operator and its tensors, for each plan we can statically derive performance factors such as per-core computation task, per-step communication volume, and memory footprint.
Second, the computation on each core in each step only consumes data from local memory, inherently preventing unpredictable memory stalls from lower-level memory.
For each operator type, we fit a linear regression model by taking factors such as total FLOPS, tensor shape, and number of steps as inputs to predict the execution latency.
Also, an interface is exposed for users to implement custom cost functions.
Lastly, the communication time is also accurately fitted by a linear regression model that takes the data transfer volume as input.

With the cost model, \oursys{} quickly examines each execution plan and choose the best candidates that sit on the Pareto-optimal trade-off curve, where each plan either runs faster than any other plans with the same or less memory footprint or uses less memory than any others with the same or lower execution time (see Figure~\ref{fig:intra_performance} in our evaluation for details). 

\begin{figure}[t]
    \centering
    \includegraphics[width=1.01\linewidth]{figures/eval_cost.png}
    \vspace{-5.5ex}
    \caption{Cost model accuracy for different operator types and shapes. Each point represents the measured vs. predicted execution time of a sub-operator.}
    \label{fig:intra_cost}
    \vspace{-3ex}
\end{figure}

\vspace{0.2em}
\noindent
\textbf{Cost model accuracy.}
To test the accuracy of the cost models, we vary the shapes of the operator and compare the predicted execution time to the actual profiled execution time. \Cref{fig:intra_cost} shows the accuracy of representative operator types. For most operators, \pname{} achieves near-perfect accuracy. The only exception is convolution, which is implemented with vendor-supplied kernels that apply some black-box optimizations. Even with slight inaccuracy, \pname{} can still find sufficiently good execution plans and outperform state-of-the-art compilers (see $\S$\ref{sec:eval_intra_op}). We envision that hardware vendors would be able to supply a perfect cost model for their kernels as they integrate \pname{} in their toolchain.

% \vspace{0.2em}
% \noindent
% \textbf{Search policy.}
% [TODO]




\vspace{0.2em}
\noindent
\textbf{Search constraints.}
In practice, a substantial portion of plans are evidently inefficient, and it is unnecessary to evaluate them with the cost model.
Thus, \oursys{} employs a rule-based approach to filter out inefficient plans, by applying two user-configurable constraints.
First, a plan utilizing too few cores will lead to compute underutilization, thus, the \textit{parallelism constraint} specifies the minimum number of cores used by an operator, filtering out plans with low parallelism.
Second, to leverage the matrix accelerator unit (e.g., AMP in IPU~\mbox{\cite{ipu_hardware}}) in each core, we may need to pad the tensor shape to align with the hardware, which wastes memory space and FLOPS.
Thus, the \textit{padding constraint} specifies the maximum padding as the ratio between the original tensor size and the padded tensor size, filtering out plans with excessive padding.
% This can introduce significant waste if the padding size is too large.
% A large padding can significantly waste memory space and FLOPS.
% To avoid inefficient padding, \oursys{} employs a rule-based approach~\cite{roller} to filter out inefficient plans. %, which typically constitute the majority of the space.
Only the remaining plans are evaluated by the cost model.
% We apply two user-configurable constraints to filter inefficient execution plans in $\S$\ref{sec:design:optimization}:
% (1) the \textit{parallelism constraint} specifies the minimum number of cores used by an operator, which filters out plans with low parallelism;
% % (2) the \texttt{compute padding constraint} specifies the maximum padding size of the AMP unit in each core;
% and (2) the \textit{padding constraint} specifies the maximum padding as the ratio between the original tensor size and the padded tensor size, which filters out plans with large padding sizes that waste both memory and FLOPS.
We examine the impact of both constraints in
\S\ref{sec:eval_intra_op}.
% We quantify the search space size reduction in Figure~\ref{fig:intra_search}. 

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/ipu-idle_tradeoff.drawio.pdf}
    \vspace{-3ex}
    \caption{Switching operator state from idle to active. There is a tradeoff between the memory footprint of idle states vs. the time of turning idle states to active states (setup time). }% Deduplicate idle operators
    \label{fig:idle}
    \vspace{-3ex}
\end{figure}


% \vspace{0.2em}
% \noindent
% \vspace{-2.5ex}
\subsubsection{Holistic Inter-operator Memory Reconciliation}
\label{subsubsec:inter-operator}
% \vspace{-0.3em}

% \newlength{\oldtextfloatsep}
% \setlength{\oldtextfloatsep}{\textfloatsep}
% \setlength{\textfloatsep}{0pt}% Remove \textfloatsep



To execute a DNN model, \oursys{} adopts the common approach of fitting multiple operators into on-chip memory, 
while only transferring the input and output data through off-chip memory.
This strategy is advantageous as adjacent operators can reuse full intermediate data in the fast on-chip memory.

Given the limited on-chip memory, each operator in \oursys{} is assigned two execution plans — one for minimum memory usage before operator execution (called \textit{idle state}) and one for minimum latency during execution (called \textit{active state}). When an operator begins to execute, a \textit{setup phase} transforms the partitioning plan from idle state to active state, i.e., by transferring the necessary data through the inter-core connection. 
This creates a tradeoff between memory usage at idle state and the overhead at the setup phase.
Figure~\ref{fig:idle} 
\hl{shows the tradeoff among different states of a MatMul operator.}

As each operator has many choices for idle and active plans, \oursys{} trades-off globally with a holistic inter-operator reconciliation policy, as shown in Algorithm~\ref{alg:inter-op}.
Initially, \oursys{} assigns the memory-efficient plan as the idle plan for all operators (line 3).
The remaining memory space after placing all operators is considered as the \textit{active memory}\footnote{\textit{Active memory} is the memory space used by the operator currently in active state, and \textit{idle memory} is the space used by operators in the idle state.}, which is used for executing the sub-operators.
\oursys{} then searches for the best execution plan by greedily trading more active memory space for \textit{idle memory} space, aiming to reduce more setup time at the cost of slightly increasing execution time.


\newcommand\mycommfont[1]{\footnotesize\sffamily\textcolor{purple}{#1}}
\SetCommentSty{mycommfont}
% \SetAlFnt{\small\sffamily}
% \newlength{\textfloatsepsave}
% \setlength{\textfloatsepsave}{\textfloatsep}
% \setlength{\textfloatsep}{0pt}
% \begin{figure}[t]
\begin{algorithm}[t]
% \footnotesize
\small
\DontPrintSemicolon
\SetAlgoNoEnd
\SetAlgoLined
% \SetAlgoHangIndent{0em}
% \Setvlineskip{-4ex}
% \SetAlgoSkip{0ex}
% \KwIn{{\it all\_ops} $\gets$ }
% \SetKwBlock{Begin}{Function}{End Function}
\SetKwFunction{FMain}{{\it get\_best\_idle\_configs}}
\SetKwProg{Fn}{Function}{:}{}
% \Begin(get\_best\_idle\_configs([[op0\_configs], [op1\_configs], ...]))
% \Fn{\FMain{[[op0\_configs], [op1\_configs], ...]}}
\Fn{\FMain{all\_ops}}
{
  \tcp{\color{purple}{start from the memory-efficient plan}}
  \For{op in all\_ops}
  {
    \textit{idle\_plan[op]} $\gets$ plan with min memory use \;
  }
  \textit{idle\_mem\_size} $\gets$ $\sum_{\textit{op} \in \textit{all\_ops}}\textit{idle\_plan[op].size}$\;
  \textit{cur\_best\_time} $\gets$ $\infty$ \;
  \While{idle\_mem\_size < max\_mem\_per\_core}
  {
    \tcp{\color{purple}{update active plan for each op}}
    \For{op in all\_ops}
    {
      \textit{active\_plan[op]} $\gets$ fastest plan that fits in mem \;
    }
    % \tcp{\color{purple}\textbf{evaluate current plan}}
    \textit{time} $\gets$ \textit{estimate\_total\_time(idle\_plan, active\_plan)} \;
    \If{time < cur\_best\_time}
    {
      % \tcp{\color{purple}\textbf{update the current best plan}}
      \textit{cur\_best\_time} $\gets$ \textit{time} \;
      \textit{cur\_best\_plan} $\gets$ \textit{(idle\_plan, active\_plan)} \;
    }
    \tcp{\color{purple}{find the best operator and increase its idle mem size}}
    \textit{best\_op} $\gets$ op with highest $-\Delta T_S /\Delta M_I$ \;
    update \textit{idle\_plan[best\_op]} with new plan \;
    update \textit{idle\_mem\_size} based on the new \textit{idle\_plan} \;
  }
  \Return{cur\_best\_plan}
}
\caption{Inter-op memory reconciliation policy.}\label{alg:inter-op}

% \afterpage{\global\setlength{\textfloatsep}{\oldtextfloatsep}}% Reset \textfloatsep

\end{algorithm}
% \vspace*{-5ex}


For each search step, \oursys{} first selects the best operator,
which has another execution plan that reduces the most setup time while adding the smallest idle space.
This plan is found by computing the ratio $\Delta T_S /\Delta M_I$ for each operator, where $\Delta T_S$ and $\Delta M_I$ are the reduced setup time and the increased idle space
(line 13).
To apply the plan change, the active memory space is subtracted by $\Delta M_I$
% After selecting the best plan, the active space is updated by subtracting $\Delta M_I$.
(line 15).
\oursys{} updates the total execution time by finding the fastest execution plan that fits in the given active memory for each operator (line 8),
and adding up the latencies of all operators (line 9).

\begin{figure*}
    \centering
    % \vspace{-1.1ex}
    \includegraphics[width=0.88\linewidth]{figures/ipu-Placement.drawio.pdf}
    \vspace{-3ex}
    \caption{Sub-tensor placement for a matrix multiplication operator on 3$\times$3 cores.}
    \label{fig:placement}
    \vspace{-3ex}
\end{figure*}

The inter-operator scheduling policy of \oursys{} can explore the complex search space with low algorithmic complexity. While there are $\prod_{i=0}^{\# ops}(op[i].num\_idle\_plans)$ idle plan combinations in total, we acquire an optimized one by searching only $\sum_{i=0}^{\# ops}(op[i].num\_idle\_plans)$ promising combinations. Given the moderate number of possible trade-off configurations, \oursys{} currently searches all steps and chooses the one that can lead to the minimum end-to-end execution time.

% \begin{algorithm}[t]
% \footnotesize
% \caption{Inter-operator memory reconciliation policy.}
% \label{alg:priority}
% \begin{algorithmic}[1]
% \Function{get\_best\_idle\_configs}{[[op0\_configs], [op1\_configs], ...]}
%     \For{op in all\_ops}
%         \State idle\_plan[op] <- plan with min memory use
%     \EndFor
%     \While{sum(idle\_plan[].mem) < max\_mem\_per\_core}
%         \For{op in all ops}
%             \State exec\_plan[op] <- fastest plan fits in mem
%         \EndFor
%         \State time <- estimate\_total\_time(idle\_plan, exec\_plan)
%         \If{time < cur\_best\_time}
%             \State cur\_best\_time <- time
%             \State cur\_best\_plan <- (idle\_plan, exec\_plan)
%         \EndIf
%         \State increment idle plan for op with highest $-\Delta T_W /\Delta M_I$
%     \EndWhile
%     \State return cur\_best\_plan
% \EndFunction
% \end{algorithmic}
% \end{algorithm}

% \vspace{-2ex}
\subsection{Mapping to the Hardware Accelerator}
\label{sec:design:hardware}
% \vspace{-0.5em}
% \setlength{\textfloatsep}{\textfloatsepsave}



The compilation approach of \oursys{} is designed to be extensible for general distributed on-chip memory-based accelerators, which can be abstracted into a unified architecture with multiple cores, each equipped with dedicated local memory and interconnected via a high-speed on-chip network.

\vspace{0.2em}
\noindent
\textbf{Abstracted device interface.}
% To facilitate adaptation to different accelerators, 
\oursys{} abstracts three key device interfaces: 
% \texttt{allocate}, \texttt{compute}, and \texttt{shift}
\textbf{(1)} \texttt{allocate} serves as a compile-time interface to allocate memory space for placing tensor partitions.
\textbf{(2)} \texttt{compute} functions as a code generation interface that emits instructions for computing a specific sub-operator on a core. By default, \oursys{} utilizes a few pre-defined code templates to generate single-core computing logic for each specific partition configuration. 
\textbf{(3)} \texttt{shift} serves as a runtime communication primitive to transmit a sub-tensor to the specified destination core.
\oursys{} leverages these interfaces to map the optimized execution plan to an accelerator.

\vspace{0.2em}
\noindent
\textbf{Sub-tensor placement.}
\oursys{} allocates the entire memory space and assigns each sub-tensor to its corresponding core. To optimize memory consumption, \oursys{} performs tensor liveness analysis to reuse the memory of precedent operators. To ensure that sub-tensors from different tensors are in the same core at each rotating step, \oursys{} arranges the initial placement of each tensor partition step-by-step by analyzing the computing order of each sub-operator and their data dependencies.
This ensures that (1) the initial placement of all sub-tensor partitions satisfies the data dependency on each core, and (2) sub-tensor partitions along each axis are in ascending order, guaranteeing that the data dependency on each core is still satisfied after each rotating step.

We show an example of placing sub-tensors for a 3$\times$3 matrix multiplication (i.e., \Cref{eqn:matmul_texpr} with $M=K=N=3$) in \Cref{fig:placement}.
Initially, all output sub-tensors ($C_j^i$) are allocated based on the partitioning plan.
Then, the first sub-tensor set $\{A^0_0, A^0_1, A^0_2\}$ is partitioned along the temporal dimension and distributed to the corresponding cores (the first row of cores).
Given the current placement of $A^0_i$ and $C^0_i$, we infer that $B_i^i$ should be placed in the first row of cores due to data dependency.
Subsequently, the remaining $B_i^j$ sub-tensors are placed sequentially in each column of cores.
Following this process, the placement of all $A_i^j$ sub-tensors can be inferred.

\vspace{0.2em}
\noindent
\textbf{Sub-operator computation scheduling.}
After the tensor placement, \oursys{} organizes the computation on each core as nested loops of interleaved \texttt{compute} and \texttt{shift} stages. Each loop corresponds to a temporal partition number.
% For example, if there are two dimensions to shift, $m$ and $n$, with $m$ shifting twice and $n$ shifting once, then there are two valid 5-time shift schedules: (1) $m$ is the inner loop, i.e., shift($m$)$\times 2\to$ shift($n$) $\to$ shift($m$)$\times 2$; and (2) $n$ is the inner loop, i.e., shift($n$) $\to$ shift($m$) $\to$ shift($n$) $\to$ shift($m$) $\to$ shift($n$).
To determine the optimal loop order, \oursys{} designates the dimension belonging to the tensor with the smaller size as the inner loop to reduce the total communication volume, as the inner loop is executed more times.
% During shifts, each core performs one round of computation on its local data.
To generate local computations for each core, \oursys{} invokes the corresponding \texttt{compute} function with the partition configuration and the tensor expression.








==> design_old.tex <==
\subsection{Spatial-Temporal Mapping Space}
\label{sec:design:space}
To map a computation, such as a DNN operator, across distributed cores, \pname{} uses a standard tensor expression to represent the operator, as described in TVM~\cite{tvm}. The expression defines the logic how each output tensor element is computed based on the input tensor values. For instance, a matrix multiplication of tensors $A$ and $B$ into $C$ expresses as follows,
\[C[m, n] \mathrel{+}= A[m, k] * B[k, n],\]
where $m$, $n$, and $k$ represent the dimension variables in both input and output tensors. The expression indicates that any value in $C$ indexed by $m$ and $n$ (e.g., $C[m, n]$) is calculated by a sum reduction over $A[m, k]$ and $B[k, n]$ for all potential indices $k$.

\hl{Similarly, \pname{} supports all operators that can be written as a tensor expression described in TVM. For example, a 2D convolution is expressed as}
$O[B, OC, OH, OW] += I[B, IC, OH+KH, OW+KW] * C[OC, IC, KH, KW]$\hl{, where B is batch size, IC/OC is input/output channel, OH/OW is output height/width, and KH/KW is kernel height/width.}

To map one operator to all cores, the tensors are partitioned across the cores and a sub-operator is composed for each core with data dependencies only on the sub-tensors assigned to it. To achieve this, \pname{} organizes all cores in a spatial-temporal space and maps all tensor partitions into it.


\vspace{0.2em}
\noindent
\textbf{Spatial mapping.}
\pname{} begins by extracting all unique dimensions present in a given tensor expression and placing them into a dimension set $S$. For example, in the matrix multiplication expression mentioned earlier, $S=\{m, n, k\}$.
If a tensor dimension is a combination of other dimensions, \pname{} selects the largest dimension to represent it. For instance, in the 1D convolution expression $O[n] += I[n + k] * C[k]$, the dimension of tensor $I$ is the sum of $n$ and $k$, with $k$ representing the kernel dimension and usually being significantly smaller than $n$ (i.e., input size). As a result, we use $n$ to represent this dimension and the dimension set becomes $S=\{n, k\}$.

To map an operator to all distributed cores, we can partition the computation along any dimensions in $S$. We use a vector of factors $F=(f_0, f_1, ..., f_n)$ to indicate the partitioning factor for each corresponding dimension in $S$. As a result, the total number of partitions is the product of all factors in $F$.
\hl{For example, a partitioning factor $F = (3, 2)$ will slice an operator with $S=\{n, k\}$ into 3*2=6 sub-operators, each of which has $S_{sub}=\{{n\over3}, {k\over2}\}$.}
We also reorganize all cores into a multi-dimensional array of shape $F$, so that each core stores one partition of the operator.
Specifically, both the input and output tensors are partitioned along $F$ and mapped to the corresponding cores. If a \hl{partitioned} dimension does not belong to a specific tensor, \pname{} automatically duplicates this tensor to all cores along this dimension.
For example, in Figure~\ref{fig:motivation_example}(b), the input tensor is partitioned along $m$, and the weight tensor lacks an $m$ dimension. Therefore, \pname{} duplicates the weight tensor along the $m$ dimension on both core 0 and core 1.
Note that if a reduction dimension\footnote{\hl{A reduction dimension is a dimension along which the input values will be reduced/summed into one output value.}} is partitioned, the result tensor will be duplicated along \hl{this partitioned} dimension on multiple cores, with each holding a partial reduction result.
Once the mapping is complete, each core holds a sub-operator that operates on only the local sub-tensors assigned to it, while still following the original computation logic.



\vspace{0.2em}
\noindent
\textbf{Temporal mapping.}
Once the spatial mapping is done, some sub-tensors may be duplicated across multiple cores to ensure local access. To address the capacity waste caused by duplication, \pname{} introduces an orthogonal partitioning mechanism called \textit{temporal mapping}, which allows a tensor to be partitioned over a group of cores and arranged in a circular ring that shifts its partitions in multiple time steps.

In temporal mapping, a tensor $T$ can be tiled along one of its dimensions over $N$ cores with a partition factor $f$. When $f=N$, the tensor is evenly partitioned into $N$ parts and forms a full shift ring to be shared over the $N$ cores in $N-1$ steps, as depicted in Figure~\ref{fig:shift}(c). If $f<N$ (assuming $f$ divides $N$), every $f$ cores will form a local shift ring, resulting in a total of $N/f$ rings. This means the tensor $T$ is duplicated in each ring for a total of $N/f$ time, as illustrated in Figure~\ref{fig:shift}(b). In an extreme case where we specify $f=1$, tensor $T$ is duplicated on every core, requiring zero shift steps, as shown in Figure~\ref{fig:shift}(a). This is also the default case after spatial mapping.

Temporal mapping differs from spatial mapping in that it can be specified individually for each tensor. 
Thus, a vector of partition factors, denoted as $F_t=(f_0, f_1, ..., f_d)$, can be further defined for each tensor for each temporal dimension, with each factor corresponding to a particular tensor dimension. 
In practice, it suffices to only perform temporal mapping for duplicated tensors to prevent unnecessary shift steps.

In light of this, \pname{} introduces a comprehensive operator partition space for distributed cores along both \hl{spatially and temporally partitioned dimensions}.
\hl{An operator will first be spatially partitioned to generate a set of spatial mapping plans. For each spatial mapping plan, a set of temporal partitioning factors can be further defined for each tensor, with each factor corresponding to a particular tensor dimension.}
A distinct partitioning plan is uniquely established by a spatial factor vector $F_s$ and multiple temporal factor vectors $F_t^i$ for each tensor $i$.
Each valid partitioning plan implies a unique execution plan that covers the mapping of each tensor to individual cores, the flow of sub-tensors across cores, and the computation of each core at a given step.
For example, if we specify the $F_s=(m:N, k:1, n:N)$, $F_t^{out}=(m:1, n:1)$, $F_t^{in0}=(m:1, k:N), F_t^{in1}=(k:N, n:1)$ for a matrix multiplication $C=A*B$, it will automatically form an $N\times N$ Cannon's algorithm~\cite{cannon} for distributed matrix multiplication, as illustrated in Figure~\ref{fig:cannon}(a).
\hl{Since \pname{} homogeneously partitions an operator across all cores, each sub-operator has exactly the same computation and communication pattern. By keeping the workloads on all cores balanced, \pname{} prevents the performance from being bottlenecked by slower threads.}

% \yiqi{for matmul(m, k, n) with output stationary cannon, $F_s=(m:N, k:1, n:N)$, \\
% $F_t^{out}=(m:1, n:1)$, $F_t^0=(m:1, k:N), F_t^1=(k:N, n:1)$}


% To generate the execution plans for one operator, we first partition the operator into spatial parts as shown in \Cref{fig:motivation_example}b, where each part is mapped to one core.
% After that, we further partition the resulting sub-operators into temporal rounds as shown in \Cref{fig:motivation_example}c.

% To abstract the above partitions, we develop the terminology shown in

% $\\$OP info:\\
% \yiqi{dim\_lengths}
% \\$[chl=dim0\_len, ker\_wid=dim1\_len, ...]$\\
% \yiqi{variable\_shapes}
% \\$[tensorA: [[chl\_idx], [ker\_wid\_idx, out\_wid\_idx]], \\
% tensorB: [[...], [..., ...], [...]]]$

% $\\$Partition info:\\
% \yiqi{num\_spatial\_partitions}
% \\$[dim0\_parts, dim1\_parts, dim2\_parts]$\\
% \yiqi{num\_temporal\_partitions}
% \\$[dim0: [tensorA\_parts, tensorB\_parts, tensorC\_parts], \\
% dim1: [tensorA\_parts, tensorB\_parts, tensorC\_parts], \\
% dim2: [tensorA\_parts, tensorB\_parts, tensorC\_parts]]$

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/ipu-factor.drawio.pdf}
    \vspace{-2.5ex}
    \caption{Illustration of temporal mapping.}
    \label{fig:shift}
    \vspace{-2ex}
\end{figure}

\subsection{Cost-aware Intra-operator Scheduling}
\label{sec:design:intra_op}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/ipu-cannon.drawio.pdf}
    \vspace{-3ex}
    \caption{Cannon Algorithm.}
    \label{fig:cannon}
    \vspace{-3.5ex}
\end{figure}

Although the aforementioned mechanism is flexible to represent all possible partitioning plans, it presents a substantial optimization space that contains numerous configurations that are either invalid or noticeably inefficient. To address this issue, \pname{} applies some explicit optimization rules as constraints during the partitioning process.  
For example, coordinating the shift of multiple tensors can lead to substantial savings in terms of both data transfer volume and computation steps. 
\hl{\pname{} first uses the constraints to filter out partitioning plans that are highly possible to be ineffective, which reduces search space size and speeds up compilation.}
To this end, we have divided our constraint rules into three categories: spatial parallelism constraints, temporal alignment constraints, and computation padding constraints. 
\hl{Then, \pname{} uses a cost model to find the optimal plans that require the least memory capacity or execution time.}

\vspace{0.2em}
\noindent
\textbf{Parallelism constraints.}
To better align with the partition size of an operator, \pname{} allows an operator to be mapped on a subset of cores, so the total number of spatial partitions in a partitioning plan could be less than the total number of available cores. 
However, utilizing too few cores for an execution plan could lead to significant inefficiencies. 
Thus, we also enforce a constraint on the ratio of idle cores, ensuring that it is less than a specified threshold, such as 5\%.

\hl{In practice, the parallelism constraint threshold can be configured by users, and \pname{} automatically relaxes the threshold for operators with no qualified plans under the given threshold. In our experiments, we set the threshold to 5\% to filter out plans utilizing less than 95\% of the cores. For small operators that cannot saturate 95\% of the cores, \pname{} will iteratively double the threshold until it finds a plan, as these small operators are rare and incur low execution overhead. This allows \pname{} to efficiently find promising plans.}


\vspace{0.2em}
\noindent
\textbf{Alignment constraints.}
To ensure that a temporal partitioning can be translated into a valid execution plan, the product of the temporal partition factors of a tensor (i.e., the total number of temporal partitions) should be a factor of the replication number caused by spatial partitioning. 
Additionally, for different tensors of an operator that share a common dimension, all their temporal factors on this dimension should be aligned. 
Thus, any pair of temporal factors should be a factor or multiple of each other. 
This approach allows each tensor or sub-tensor to flow across cores at a different pace, while ensuring that corresponding tensor partitions can meet at the same time step on a specific core.

For instance, consider the variant Cannon matrix multiplication illustrated in Figure~\ref{fig:cannon}(b), where tensor B has a temporal partitioning along dimension $k$ for an $N/2$ factor (i.e., $F_s=(N, N)$, $F_t^0=(1, N)$, and $F_t^1=(N/2, 1)$). As a result, tensor B is duplicated twice and shifted once every two time steps, while tensor A is still shifted for each step.

%\yiqi{The above scenario partitions one shift dimension with length $N$ into two shift dimensions with lengths $N/2$ and $2$. Thus, we can choose from two nested loop options with either of the shift dimensions being the outer loop. On execution, both tensors shift one step per iteration transition of the $N/2$ loop, while only tensor A shifts one step per iteration transition of the loop with length $2$, as shown in \Cref{fig:overview}(b)}

\vspace{0.2em}
\noindent
\textbf{Computation padding constraints.}
In order to take advantage of the fast matrix unit present in each core, such as the AMP in IPU, it is often necessary to pad the matrix shape of a sub-operator to a multiple of the matrix unit size. However, if a partitioning plan leads to a sub-operator shape that requires too much padding, significant amount of wasted computation occurs. Thus, \pname{} restricts the padding size to be within a small ratio when compared to its tensor size.

\hl{The padding constraint is a common practice for DNN compilers\mbox{~\cite{roller,tensorir}}. T10 leverages a similar approach by exposing the constraint to the user as a tunable compiler hyper-parameter. A smaller padding constraint helps quickly filter out inefficient partitioning plans, while a larger padding constraint includes more opportunities to find better partitioning plans at a cost of longer compilation time.
In our experiments, we use a default value that allows at most 25\% padding size compared to the tensor size. If a very small operator has no plans that saturate 75\% of the SIMD width, T10 iteratively doubles the padding constraint until it finds a plan.}



% \yiqi{Product of temporal\_parts per tensor for all dims is a factor of its number of replicas. (e.g., 8 cores cannot evenly hold 7 pieces)}

% \yiqi{The temporal\_parts per dim for all tensors must be factor or multiple of each other. (e.g., dividing 2 tensors along the same dim into 3 and 4 pieces respectively will result in unaligned shifts)}



\vspace{0.2em}
\noindent
\textbf{Plan selection guided by cost model.}
After applying the constraints mentioned above, there still remain a significant number of valid mapping plans for each operator. Thus, \pname{} further selects the optimal candidate plans by taking advantage of the unique feature of DSM-based architecture, which allows for the easy derivation of an accurate cost model. This is due to the inherent execution patterns that facilitate accurate performance prediction. Specifically, the explicit separation of computation and communication phases in the execution model, such as BSP, allows for the natural modeling of the overall latency independently. Furthermore, the computation on each core in each execution step only consumes data from local memory, which inherently prevents unpredictable memory stall behaviors from lower-level memory. In the communication phase, the time taken for data transfer is highly related to the transfer volume, which can be easily modeled by a linear regression model for a specific accelerator. Lastly, the synchronization overhead at each iteration is deterministic and relatively short compared to computation and communication time. Based on these observations, we can estimate the memory utilization and execution time for each plan. Specifically, the memory consumption is equivalent to the sub-tensor size, which can be directly inferred given a partition plan. For the computation time of a sub-operator, we default to fitting a linear regression model that takes the total flops of a sub-operator as a variable for each operator type. For some special operator implementations, we extend the regression model by adding more critical factors such as tensor size and number of loops. We also expose an interface for users to implement a custom cost function for custom kernels. 
Using the cost model, \hl{T10 analyzes the sub-operator size and execution time for each operator given a specific partitioning plan.}
It can efficiently examine each valid plan and choose the best candidates that sits in the best memory and execution time trade-off line, as illustrated by the green points in Figure~\ref{fig:overview}(b).

\subsection{Inter-operator Memory Reconciliation}
\label{sec:design:inter_op}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/ipu-idle.drawio.pdf}
    \vspace{-1.5ex}
    \caption{Deduplicate idle operators.}
    \label{fig:idle}
    \vspace{-3ex}
\end{figure}

DSM accelerators usually have sizable on-chip memory but comparatively limited off-chip memory bandwidth. 
\hl{Meanwhile, the data sharing between adjacent operators is very frequent, as many operators take the output of the preceding operator as input. In fact, one benefit of DSM-based accelerators over GPUs is that its large on-chip memory can fit a chain of operators, so the adjacent operators can share data on chip. On the contrary, the GPU often cannot even fit one single operator in its on-chip memory, so adjacent operators can only exchange data through the slow off-chip memory.
}
To execute a complete DNN model, \pname{} follows the common approach which fits all operator parameters of the model into the on-chip memory while allocating the off-chip bandwidth solely for transferring input data and output results.

\vspace{0.2em}
\noindent
\textbf{Idle and active operator state.}
For each operator, \pname{}'s intra-operator scheduling can generate multiple optimal plans, each representing a different trade-off between memory consumption and execution latency. For example, a plan may use more memory space for storing some tensor replicas to trade off for lower latency due to fewer shifting steps. With the fast inter-core connection of DSM architecture, two partitioning plans can be assigned for each operator - one for minimum memory usage before the operator execution (called idle state) and one for fast execution time during the execution (called active state). 
When an operator begins to execute, a warm-up phase transforms the partitioning plan from idle state to active state, i.e., by transferring the necessary data through the inter-core connection. Figure~\ref{fig:idle} illustrates a matrix multiplication operator and its different states. 
In the idle state, the partitioning plan with less duplication is chosen to save memory consumption. During the warm-up stage, a few sub-tensors are transferred to other cores to change into another partitioning plan, which involves duplicating one input tensor for multiple times but leads to faster execution time due to its zero shift step requirement.
\hl{Since both the idle and active plans are candidate plans generated by intra-operator scheduling, and they share the same spatial mapping, the only difference between the two plans is that they duplicate the tensors differently. Thus, \pname{} makes a multi-broadcast plan like the one shown in Figure\mbox{~\ref{fig:idle}} by comparing the placement of each tensor between both plans.}

\hl{Consequently, there is a trade-off between the memory usage at idle state and the overhead at warm-up phase. If the memory is very limited, data will be significantly deduplicated at idle state, and the warmup overhead can be high. Thus, \pname{} employs a holistic memory reconciliation mechanism to consider this trade-off and optimize the end-to-end execution time.}


% \begin{algorithm}[t]
% % \footnotesize
% \caption{Inter-operator memory reconciliation policy.}
% \label{alg:priority}
% \begin{algorithmic}[1]
% % \State priority\_list = [wl.priority for wl in workload\_list]
% \Function{get\_best\_idle\_configs}{[[op0\_idle\_configs], [op1\_idle\_configs], ...]}
% % https://drive.google.com/file/d/1gcI2pbnteWPXEvKO05_x6oUnLR3acn6l/view?usp=sharing   Inter OP Tradeoff
%     \State start from idle configs without duplication for all ops
%     \While{idle space < on-chip memory}
%         \For{all ops}
%             \State apply fastest exec plan w/o mem overflow
%         \EndFor
%         \State record total latency
%         \State apply config increment step with highest 
%         \State $delta(warmup\_time) / delta(idle\_mem)$
%     \EndWhile
%     \State return best\_configs with lowest total latency
% \EndFunction
% \end{algorithmic}
% \end{algorithm}

% \setlength{\textfloatsep}{7pt}
\begin{algorithm}[t]
\footnotesize
\caption{Inter-operator memory reconciliation policy.}
\label{alg:priority}
\begin{algorithmic}[1]
% \State priority\_list = [wl.priority for wl in workload\_list]
\Function{get\_best\_idle\_configs}{[[op0\_configs], [op1\_configs], ...]}
    \For{op in all\_ops}
        \State idle\_plan[op] <- plan with min memory use
    \EndFor
    \While{sum(idle\_plan[].mem) < max\_mem\_per\_core}
        \For{op in all ops}
            \State exec\_plan[op] <- fastest plan fits in mem
        \EndFor
        \State time <- estimate\_total\_time(idle\_plan, exec\_plan)
        \If{time < cur\_best\_time}
            \State cur\_best\_time <- time
            \State cur\_best\_plan <- (idle\_plan, exec\_plan)
        \EndIf
        \State increment idle plan for op with highest $-\Delta T_W /\Delta M_I$
    \EndWhile
    \State return cur\_best\_plan
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{figure*}
    \centering
    \includegraphics[page=5,width=0.9\linewidth]{figures/ipu-Placement.drawio.pdf}
    \vspace{-2.5ex}
    \caption{Sub-tensor placement for a 3$\times$3 Cannon algorithm.}
    \label{fig:placement}
    \vspace{-2ex}
\end{figure*}


\begin{figure}[t]
    \centering
    \includegraphics[page=5,width=0.9\linewidth]{figures/ipu-ComputeSet.drawio.pdf}
    \vspace{-3ex}
    \caption{IPU kernel code example.}
    \label{fig:codegen}
    \vspace{-1ex}
\end{figure}

\vspace{0.2em}
\noindent
\textbf{Holistic memory reconciliation.}
During the execution of the model, only one operator can be executed at any given time, while other operators are in the idle state and only occupy a portion of the idle memory space to store their tensors. As each operator could have different choices for the idle and active plans, a global optimization execution plan is needed to reconcile each operator's trade-off space holistically. \pname{} achieves this by deciding on an optimal memory size allocation for idle memory and active memory. Algorithm~\ref{alg:priority} presents \pname{}'s memory reconciliation process. Initially, \pname{} assigns the partitioning plan with zero duplication as the idle plan for all operators. The remaining memory space after placing all the idle operators is considered the active memory, which will be used for executing each operator. \pname{} searches for the best execution plan by greedily trading more active space for idle space, aiming to reduce more warm-up time (due to more duplication) at a cost of only slightly increasing execution time (due to fewer duplications). For each searching step, \pname{} first selects the best operator and its partitioning plan that can reduce the most warm-up time by adding the smallest idle space. This plan is found by calculating the ratio of $\Delta T_W /\Delta M_I$ for each operator, where $\Delta T_W$ and $\Delta M_I$ are the reduced warm-up time and increased idle memory space, respectively, if the next partitioning plan is chosen for an operator. After selecting the best plan, the active space is updated by subtracting $\Delta M_I$. Then, \pname{} calculates the new execution time by enumerating each operator to find the fastest execution plan that can fit in the given active memory space and accumulates its latency into the total execution latency. 
\hl{If there is no way to fit all operators, \pname{} will not find a valid end-to-end plan to report.}
Conclusively, while there are $\prod_{i=0}^{\# ops}(op[i].num\_idle\_plans)$ idle plan combinations in total, we acquire \hl{an optimized} one by searching only $\sum_{i=0}^{\# ops}(op[i].num\_idle\_plans)$ promising combinations.
Given the moderate number of possible trade-off configurations, \pname{} currently searches all steps and chooses the one that can lead to the minimum end-to-end execution time.



% For elementwise and pure-reduction OPs (overall duplication is always low for any spatial partition plans, and at least one var has all dims), do not change partition configuration if reuse.

% Due to the limited off-chip memory bandwidth of IPU and the large on-chip memory, the most common usecase of IPU is that we put the entire model parameters 
% for all operators inside the on-chip memory, while reserving the off-chip link exclusively for transferring input data and output results. 
% Thus, at any time of the execution there is only one operator being actively executed, while other idle operators still occupy the on-chip memory to store their parameters.
% However, some of the promising candidate plans we found for each operator in \Cref{sec:design:intra_op} employ a moderate amount of duplication to improve the execution FLOPS. 
% Thus, we can further deduplicate the parameters when their operators are idle to save more on-chip memory.


\subsection{Hardware Abstraction}
\label{sec:design:hardware}

% \setlength{\textfloatsep}{2em}


\noindent
\textbf{\pname{} hardware interface.}
% The optimal partitioning plan for an end-to-end model achieved by \pname{} above is a configuration intended to be mapped to general DSM-based architectures.
To facilitate adaptation to various DSM-based accelerators, \pname{} abstracts three key device interfaces: \texttt{allocate}, \texttt{compute}, and \texttt{shift}.
\texttt{allocate} serves as a compile-time interface that enables \pname{} to allocate memory space for placing tensor partitions beforehand. \texttt{compute} functions as a code generation interface that emits instructions for computing a specific sub-operator on a core. By default, \pname{} utilizes a few pre-defined code templates to generate single-core computing logic for each specific partition configuration.
Lastly, \texttt{shift} serves as a runtime communication primitive that offers a memory-efficient method for transferring a tensor from one core to another.
% Note that directly copying a tensor across cores needs a memory buffer on both the sender and receiver sides, resulting in significant waste of on-chip memory. \pname{} provides a default implementation of \texttt{shift} by dividing a tensor into sufficiently large chunks that can saturate the transferring bandwidth. The appropriate chunk size is tuned only once for a specific device.

\vspace{0.2em}
\noindent
\textbf{Sub-tensor memory allocation.}
By utilizing the above hardware interface, a concrete execution plan is generated from the partition configuration. At compile-time, \pname{} pre-allocates the entire memory space and assigns each sub-tensor to its corresponding core. To optimize memory usage, \pname{} performs a tensor liveness analysis to reuse the memory of precedent operators. To ensure that sub-tensors from different tensors are co-located in the same core at each shift step, \pname{} carefully arranges the initial placement of each tensor partition based on their dependencies with others.

As an example, the process of placing sub-tensors for a 3$\times$3 Cannon matrix multiplication is illustrated in \Cref{fig:placement}. Initially, all output sub-tensors ($C_j^i$) are allocated based on the partitioning plan. The first sub-tensor set (i.e., $A^0_0, A^0_1, A^0_2$) is then partitioned along the temporal dimension and distributed to the corresponding cores (the first row of cores). Given the current placement of $A^0_i$ and $C^0_i$, we infer that $B_i^i$ should be placed in the first row of cores due to data dependency. Subsequently, the remaining $B_i^j$ sub-tensors are placed sequentially in each column of cores. Following this process, the placement of all $A_i^j$ sub-tensors can be inferred.
% Note that such placement process is general to be applied to various partition plans.

\vspace{0.2em}
\noindent
\textbf{Sub-tensor compute scheduling.}
% After the tensors are placed, 
\pname{} arranges the computation on each core as nested loops of interleaved \texttt{compute} and \texttt{shift} stages. Each loop corresponds to a temporal partition number.
% For example, if there are two dimensions to shift, $m$ and $n$, with $m$ shifting twice and $n$ shifting once, then there are two valid 5-time shift schedules: shift(m)$\times2\to$ shift(n) $\to$ shift(m)$\times2\to$ or shift(n) $\to$ shift(m) $\to$ shift(n) $\to$ shift(m) $\to$ shift(n).
To determine the optimal loop order, \pname{} designates the dimension belonging to the tensor with the smaller size as the inner loops to reduce the total communication volume, as the inner loops are executed more times.

% During shifts, each core performs one round of computation on its local data. To generate local computations for each core, \pname{} invokes the corresponding \texttt{compute} function by taking the partition configuration and tensor expression as inputs. 



% for the shift stage,  determine the order of nested loops for all shifted dimensions. For instance, if there are two dimensions to shift, $m$ for 2 times and $n$ for 1 time, then there are two valid 5-time shift schedules: shift(m)$\times2$->shift(n)->shift(m)$\times2$ or shift(n)->shift(m)->shift(n)->shift(m)->shift(n). In practice, we designate shifts with smaller tensor sizes as inner loops to decrease the total shift volume.






\subsection{Put Them Together}
\label{sec:design:put_together}

\hl{For intra-operator scheduling, \pname{} enumerates the spatial-temporal partitioning plans for an operator as follows. First, the spatial partitioning space is determined by the available number of cores. \pname{} enumerates all spatial partitioning plans such that the number of spatial partitions is no greater than the total number of available cores. It also applies the parallelism constraint to filter out the spatial plans that use too few cores (i.e., have too few partitions). After spatial partitioning, some parts of the tensors may be duplicated across multiple cores for local access. Hence, for each spatial partitioning plan, \pname{} enumerates the corresponding temporal partitioning plans that satisfy the alignment constraint and the padding constraint. This gives a set of valid spatial-temporal partitioning plans for this operator. Then, \pname{} leverages the cost model to estimate the memory consumption and execution time of each spatial-temporal plan, and keeps only the Pareto-optimal plans.}

\hl{By combining intra and inter-operator scheduling, \pname{} aims to solve the fundamental problem on optimizing the trade-offs between memory consumption and execution efficiency for each operator, which forms a combinatorial optimization space.
The key insight in \pname{} is to use an aligned "cost-efficient metric" to unify the trade-off spaces in each individual operator. The metric defines how much latency can be reduced by giving a certain memory space for each operator. By leveraging such aligned metric, \pname{} is able to separate the problem into local optimizations and global optimizations. Locally, it generates the most cost-efficient plans of each operator under variant memory requirements. Globally, it decides which plan should be used for each operator by considering the global cost-efficiency i.e., end-to-end latency with a given memory budget. This leads to our efficient greedy memory reconciliation algorithm for navigating the large search space.}


==> idea.tex <==
\section{Core Idea of \pname{}}
\label{sec:idea}



Instead of relying on global memory abstraction, our approach is to partition each operator into sub-operators, which collaboratively hold the entire tensor data across all cores, as depicted in \Cref{fig:save_mem}(c). Moreover, to prevent data duplication, the data used by a group of sub-operators can be distributed across multiple computing rounds. Consequently, one piece of data can be temporally shared among multiple sub-operators on multiple cores by shifting through the inter-core links. As a result, global memory abstraction is no longer necessary, freeing up a large portion of local memory for sub-operator execution. This method could also reduce data fetching from remote cores, as part of the data is explicitly placed in the local memory of each core.

For instance, to compute the MatMul in \Cref{fig:motivation_example}(a), we first spatially partition the operator into two cores in \Cref{fig:motivation_example}(b), where the second input tensor (weight) is duplicated in both cores. At this point, the on-chip memory is insufficient to hold all the partitioned variables. While previous works would use virtual global memory to de-duplicate the weight at the cost of an extremely small sub-operator size, we can improve by further partitioning the operator temporally into 2 rounds in \Cref{fig:motivation_example}(c). Thus, each core holds half of the duplicated weight and completes half of its computation per round. Between rounds, the cores shift their half-weight parts to the next cores. After all rounds, all cores complete their computation by going through all half-weight parts. In this solution, each partition of the shared weight is stored in at least one core at any time, eliminating the need for a global memory to store the shared data, which achieves the largest possible sub-operator size.

\vspace{0.2em}
\noindent
\textbf{Intra-operator trade-off.}
Partitioning an operator into more cores or more computation rounds offers a trade-off between duplication and data transfer volume. For instance, slicing and shifting a small tensor over multiple rounds may save little memory space while incurring considerable synchronization overhead. On the other hand, slicing a large tensor could save significant memory with a relatively minor cost of communication. Simultaneously, the trade-off is also influenced by the local computation efficiency of different sub-operator shapes. For example, the AMP unit in IPU prefers a longer input dimension to amortize the weight-reloading overhead. \Cref{fig:shape_example} illustrates an improved partition plan compared to \Cref{fig:motivation_example}, which enables higher FLOPS by increasing the input dimension length. However, it also increases duplication by copying the 8-element output instead of the 4-element weight. This means more data must be shifted per round to eliminate duplication, resulting in higher latency. Therefore, an effective evaluation method is necessary to determine the optimal trade-off (\S\ref{sec:design:intra_op}).
% by considering all factors .

\vspace{0.2em}
\noindent
\textbf{Inter-operator trade-off.}
\hl{Our designs are driven by a singular objective: best utilizing the on-chip memory. This is motivated by our key observation that DSM-based architecture has fundamentally changed the compiler optimization trade-off space: from optimizing data reuse to improving memory utilization.}
Due to the limited off-chip memory bandwidth of DSM accelerators, the common practice is to place all operators in the on-chip memory to avoid off-chip memory access during computation. To further improve memory utilization, tensors in the on-chip memory are reused as much as possible. For example, weights can be reused across inference batches, and activation tensors from producer operators can be reused by consumer operators.
\hl{If one operator uses the output tensor of the preceding operator as its input tensor, this tensor can stay in the on-chip memory to reduce expensive off-chip data transfer.}

This pattern introduces two additional trade-off decisions.
% First, given that different operators may have different intra-operator trade-off ratios (i.e., latency reduced by increasing the same memory capacity),  Therefore, we must globally consider the memory space allocation for each operator to maximize overall efficiency.
First, some operators benefit more from data duplication, while some benefit less (e.g., duplicating small operators greatly reduces synchronization overhead with little memory capacity overhead). Thus, we must globally consider the trade-off between data duplication and data transfer for all operators to maximize overall efficiency.
\hl{Therefore, instead of deliberately minimizing the data transfer overhead, we holistically optimize the end-to-end execution latency under the constraint of on-chip memory capacity.}
Second, data duplication may be unnecessary when the operator is not executing. 
\hl{Under this scenario, we want to reserve more memory for the currently active operator while keeping other operators in the limited on-chip memory.}
Each operator can be stored in a memory-efficient plan (e.g., no duplication) when idle and switch to a compute-efficient plan (with duplication) during execution at the cost of a warm-up process to switch between the plans. 
This offers a more complicated trade-off across operators among data duplication, data transfer, and warm-up (\S\ref{sec:design:inter_op}).




% \subsection{Data Transfer and Sub-operator Shape Overhead}
% \label{sec:idea:core_idea_overhead}

% While in IPU data transfer cannot be overlapped with computation, more data transfer inevitably increases the total execution latency.
% Thus, when using the above solution for complex tensor operators with multiple dimensions, we must carefully trade-off between duplication and data transfer.
% For example, we save little memory while causing considerable synchronization overhead by slicing and shifting a small tensor.
% However, by slicing and shifting a large tensor, we may save much more memory while causing only slightly more latency overhead than small-tensor cases.
% Thus, this trade-off space must be well handled for efficient compiling.

% Meanwhile, as discussed in \Cref{sec:background:many_small_cores}, to maximizes the FLOPS performance of the systolic arrays in IPU cores, we should make the inputs and outputs of sub-operators long enough to amortize the weight-reload overhead, for systolic-array operators like MatMul and convolution.
% % and the temporal partitions described above, IPU sub-operators per round per core rarely have large sizes.
% % Similar to MXU and TensorCore, the AMP unit in IPU uses a systolic array to accelerate MatMul, whose performance may be impacted by the shape of sub-operator \cite{tpu_supercomputer}.
% % When using a systolic array for MatMul, the program first loads the second input matrix, called weight, onto the processing elements (PE) inside the array.
% % Then, the program simultaneously pushes and first input matrix into the array and pops the output matrix from the array, for a duration determined by the operator shape and size.
% % When loading weights, the systolic array is not doing meaningful computation.
% However, given that sub-operator sizes are limited by on-chip memory, we can only leverage the shape of sub-operators to maximize weight reuse in most cases, which may also cause side effects.
% % of limited sizes, weight loading gets more frequent and results in lower performance.
% % To show this effect, we profile the performances for sub-operators with different input/output lengths in \yiqi{}.
% % Under extremely short lengths, the average FLOPS is only 50\% of the advertised peak performance, assuming no padding or idleness occurs.
% Comparing \Cref{fig:shape_example} to the partition plan in \Cref{fig:motivation_example}, we observe that \Cref{fig:shape_example} enables higher FLOPS by increasing the input/output length.
% However, it also magnifies the duplication by copying the 8-element output instead of the 4-element weight. 
% To eliminate the duplication in \Cref{fig:shape_example}, we need to shift more data per round, resulting in higher latency.
% Thus, a universal criterion that takes all factors into account is critical for a holistic consideration between trade-off decisions.



% \subsection{Inter-operator Trade-off}
% \label{sec:idea:inter_operator_tradeoff}

% As discussed in \Cref{sec:background:large_memory}, given the limited off-chip bandwidth of DSM devices, we reduce the pressure on it by improving the data reuse inside the chip, and this requires the on-chip memory to concurrently hold the data belongs to multiple operators.
% For example, one common usecase of Graphcore IPU is that we statically put the parameters of some or all layers in a DNN model into the chip, so multiple inference batches can reuse the parameters.  
% %However, if one single operator is not large enough to use the entire on-chip memory, we then improve data reuse by putting multiple consequent operators into the chip.
% Also, we may reuse the output of the previous operator as the input of the next operator, as it is common in DNN models that each layer uses the activation outputs of the previous layer as the inputs.
% %In the first case, for an inter-operator transition without idleness, all data of the next operator must be ready on chip before the current operator ends. 
% %Thus, inputs of the previous operators should not be discarded even after operator completions, as they may be used in the future. For example, in DNN inference cases, the same model weights may stay on the IPU forever, so inputs of different batches can be directly applied to the weights on their arrival. 
% Thus, most operators demand zero off-chip bandwidth, as their inputs are already on chip when they start, and their outputs are immediately reused by the next operator.
% % Thus, DSM accelerates working in this pattern only requires negligible off-chip bandwidth.

% However, since the chip must concurrently hold all the data of multiple operators to enable this work pattern, two additional trade-off complexities are introduced.
% First, while operators with more internal data reuse may be benefited more by additional duplication (more total latency reduction at the same data size increment), other operators may be less sensitive to it.
% Thus, we must globally consider which operator brings the most latency reduction using the same additional memory space.
% Second, there is less need to duplicate the data for an operator outside its actual execution.
% Thus, each operator may be of a cold data size when it is idle, then it duplicates and expands to hot data size just before its execution, at cost of the time spent on warmup.
% This pre-execution duplication process is also a part of the trade-off between data duplication and data transfer/warmup.

==> intro.tex <==
\section{Introduction}
\label{sec:introduction}

Deep learning accelerators, such as GPUs and TPUs, are widely recognized for their exceptional computing throughput (e.g., hundreds of Tera-FLOPS), making them ideal for handling large-scale models and high-dimensional data in deep learning. Such effectiveness is largely attributed to their massive parallel cores and specialized accelerator units, e.g., TensorCore. However, to saturate the high computing throughput, they usually require a high-throughput memory system, e.g., a large shared memory with multi-hierarchical cache layers in accelerators. 
Also, an efficient deep learning compiler~\cite{ansor, roller} is necessary to optimize data reuse across the memory hierarchy, ensuring the computing units are fully utilized. This combination of hardware and software design often yields orders of magnitude higher performance than traditional CPUs for critical deep learning operations, including matrix multiplication and convolution.%, and end-to-end model computation.

Despite the success of existing accelerators, the constantly increasing demand for processing large deep-learning models with higher computation throughput presents a significant challenge to the underlying memory system. 
To address this challenge, the community is exploring a more scalable architecture with fully distributed memory. 
\hl{Distributed (shared) memory-based (DSM) architectures have emerged as a promising solution in both industry and academia due to their ability to overcome the memory limitations posed by shared memory-based architectures such as GPUs. Notable commercial products in this field include the the Graphcore IPU\mbox{~\cite{ipu2}}, SambaNova SN10\mbox{~\cite{samba}}, Tenstorrent Grayskull\mbox{~\cite{tenstorrent}}, and Cerebras WSE\mbox{~\cite{wse2}}.}
% such as the Graphcore IPU~\cite{ipu2}, SambaNova SN10~\cite{samba}, Tenstorrent Grayskull~\cite{tenstorrent}, and Cerebras WSE~\cite{wse2}.
% \todo{verify this and add reference (TSP uses one global partition of on-chip memory)} 
Rather than relying on shared-memory architecture, they typically associate each computation core with local memory, and connect the cores via a high-bandwidth on-chip network, creating a large aggregated on-chip memory (Figure~\ref{fig:compare_arch}). 
\hl{It is worth noting that even the latest GPU, NVIDIA H100\mbox{~\cite{h100}}, has begun incorporating elements of DSM-architecture to facilitate interconnecting shared memory across multiple stream multiprocessors, thereby enabling higher computational scalability.}
However, this unique architecture renders previous deep learning compilers designed for shared-memory architectures, which cannot fully leverage the new architecture's scalability, resulting in significant memory waste (\S\ref{sec:motivation}).

Designing a deep learning compiler for distributed memory-based accelerators presents several unique challenges. First, due to the absence of global shared memory, it is necessary to partition the operators, along with their input and output tensors, into sub-operators that can operate independently on each core with only local memory access. Second, as the local memory on each core is mostly on-chip memory, the aggregated memory capacity is considerably smaller than the off-chip memory. Thus, the compiler must effectively utilize the limited memory capacity to support a model size as large as possible, without compromising on computing performance. This optimization goal differs fundamentally from that of existing compilers that primarily focus on maximizing memory access throughput.
Third, given that there is usually a trade-off between memory consumption and computation performance for each operator, an end-to-end model compilation must consider the trade-offs among all operators, generating a combinatorial optimization space that is infeasible to solve using existing compilers.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.89\linewidth]{figures/ipu-compare_arch.drawio.pdf}
    \vspace{-2.5ex}
    \caption{Comparison of TPU, GPU, and IPU chips.}
    \label{fig:compare_arch}
    \vspace{-3ex}
\end{figure}

In this paper, we present \pname{}, a deep learning compiler for end-to-end model compilation on distributed memory-based accelerators.
%while minimizing memory usage. 
The design of \pname{} is based on three key insights. First, as deep learning operators can typically be expressed in tensor expressions, the individual operator can be automatically partitioned into independent sub-operators by analyzing their data dependency from the expression and performing necessary data duplication across sub-operators. Second, to reduce the overall memory footprint on distributed memory architecture, we can explore a new trade-off space by trading more inter-core data exchange for reduced memory footprint, thanks to the high-speed inter-core connections. Third, the distributed memory architecture implies a new computation model that separates computation and communication into two distinct stages. This presents an opportunity for a compiler to design an accurate cost model for estimating the performance of each possible execution plan, leading to an efficient approach to determine the optimal end-to-end execution plan from the huge optimization space.

With the aforementioned insights, \pname{} constructs a comprehensive spatial-temporal optimization space that enables an operator to be partitioned into independent sub-operators and mapped onto individual cores. This provides the flexibility for \pname{} to trade-off between memory usage and communication overhead. To decide the most suitable partitioning plans, \pname{} designs a general cost model that utilizes the characteristics of distributed memory architecture to estimate the memory footprint and execution time of each plan. \pname{} employs a cost-aware operator scheduling process to generate a range of execution plans with varying memory footprint requirements. In consideration of the holistic model scheduling, \pname{} provides each operator with the ability to switch between memory-efficient and compute-efficient plans during execution. \pname{} then applies a holistic reconciliation process to identify the optimized end-to-end execution plan that can fit the entire model within a given device memory capacity. After that, with a set of abstracted device interfaces, \pname{} translates the execution plan into a specific execution program, consisting of nested loops over computation and shift-based communication stages across all cores.

We implement \pname{} in 10K lines of code with Python, including the execution plan optimization and kernel code generation. 
We conduct our evaluation using various types of DNN models, such as CNNs, transformers, and vision transformers, with different batch sizes. These models are compiled by \pname{} \hl{in inference mode} and evaluated on a real distributed memory-based accelerator - Graphcore IPU Mk2 chip, as well as its variants by configuring its available cores and memory capacity.
Our evaluation shows that \pname{} not only outperforms state-of-the-art DNN compilers and vendor-specific libraries by up to 5.2$\times$, 
but also allows for much larger models and operator sizes.
%e.g., with up to a \todo{xxx} improvement. 
More importantly, \pname{} is the first to provide 
%a comprehensive optimization space and 
an end-to-end compilation approach for distributed memory-based accelerator architectures. 
%By leveraging such flexibility, 
\pname{} generalizes the classic distributed matrix multiplication approach (i.e., Cannon's algorithm~\cite{cannon}) for general tensor computation with 
distributed on-chip memory architectures. We wish our systematical approach could inspire and accelerate the design of more scalable 
distributed memory-based accelerators in the future.

% AI chip design is all about how to allocate the limited chip area to different logics: compute, memory, and communication.

% Given that the computation is orders of magnitude faster than the off-chip memory, there  are generally two different design choices: the first one is to use multiple memory layers to cache the input data and reuse data access at higher-level memory. Significant portion of logics are used to implement the cache and its consistence protocol. Inter-core communication has to go through the low-level memory layers.

% Another recent direction chooses to reserve all the on-chip area besides the computation area to the local memory and an simple on-chip network. This design results in a very larger on-chip memory (e.g., near 1GB) and similar computing flops. It provides additional advantage in processing memory-intensive workloads than GPUs. 

% However, given its distinct hardware trade-off with GPUs, existing software stack (compiler or framework) usually fail to utilize the computing resource efficiently (Some measurements here)

% 1) Existing AI compilers mostly designed for GPU-like shared-memory architecture, optimizing for the  off-chip memory access, e.g., e2e latency depends on the tile configuration for data reuse.

% 2) Distributed algorithm designed for distributed servers, optimizing for inter-server communication, 
%  e.g., e2e latency depends on communication overhead. 

% In contrast, the DSM architecture has comparable computation flops, very fast inter-core communication, but very limited memory. 

% Insights: focus on efficiently utilize memory capacity, without affecting computation and communication performance. 

% Observation: 
% 1) Computation can be partitioned into multiple iterations, and the data is distributed on multiple cores, with each step shuffling a portion with other cores.

% 2) Data is only need to mapped to cores before the computation, due to the fast inter-connection. 

% 3) One operator can contribute some space to another one for better overall efficiency.

% => form a comprehensive and complicated optimization space.  

% Solution insights:

% Tensor computation inherent a regular pattern: ?

% Memory and communication can be accurately analyzed.

% Method: 
% 1) Zero-duplication: cold start; 
% 2) runtime fast remapping: leverage fast on-chip-network -> need measure 
% 3) efficient shuffling: core mechanism


\begin{figure}[t]
    \centering
    \includegraphics[width=0.89\linewidth]{figures/ipu-compare_arch.drawio.pdf}
    \vspace{-2.5ex}
    \caption{Comparison of TPU, GPU, and IPU chips.}
    \label{fig:compare_arch}
    \vspace{-3ex}
\end{figure}

==> intro_new_bak.tex <==
\section{Introduction}
\label{sec:intro}

Deep learning accelerators, such as GPUs and TPUs, are widely recognized for their exceptional computing throughput, e.g., hundreds of Tera-FLOPS facilitated by their high-performance parallel computing units like TensorCores~\cite{a100, h100, tpu_supercomputer}. This makes them ideal for handling the increasing demand for processing larger deep learning models. 
To saturate the computing throughput, such accelerators usually require a high-bandwidth memory system, e.g., hierarchical cache layers on top of a large off-chip memory like HBM~\cite{hbm}, to feed data to the computing units in time.
However, with the increasing computing FLOPS of the accelerator chip, the computing throughput is growing significantly faster than the memory bandwidth. As a result, the deep learning workloads quickly hit the memory bandwidth wall~\cite{}. 
% However, with the increasing computing FLOPS of TensorCore, the computation throughput is growing significantly faster than the memory bandwidth growth in recent generation of GPUs, leading the deep learning workload quickly hitting the memory wall\cite{}. 

% To continue scaling up the effective computing FLOPS, recent accelerator designs have been actively exploring innovative ways to increase the on-chip memory capacity, which improves the on-chip data reuse of the deep learning workloads and reduces off-chip memory bandwidth requirement. [Yuqi: TODO]

% First, the on-chip memory capacity has been increasing to provide significantly higher memory bandwidth than the off-chip HBM.
% Second, fast inter-core connections are introduced to exchange data across cores directly without going through the off-chip memory system. This not only increases the effective on-chip memory capacity but also enables dataflow programming model for reduced off-chip memory bandwidth requirement (see~$\S$\ref{sec:xxx}).
To continue scaling up the effective computing FLOPS, recent accelerator designs actively explore innovative architectural changes to alleviate memory pressure. 
Among them, two fundamental changes are becoming a mainstream trend:
(1) enlarging the on-chip memory capacity to provide significantly higher aggregated memory bandwidth;
and (2) introducing fast inter-core connections that allow data to be exchanged across cores directly without going through the off-chip memory system.
This architectural paradigm is not only embraced by an emerging set of new deep learning accelerators like Graphcore IPU~\cite{ipu2}, SambaNova SN10~\cite{samba}, Tenstorrent Grayskull~\cite{tenstorrent}, Cerebras WSE~\cite{wse2}, but also integrated into the latest GPU architectures, e.g., NVIDIA H100~\cite{h100}, by introducing an on-chip connection among the shared memory of multiple stream multiprocessors.

From a computational perspective, such change essentially transforms the memory architecture from uniform memory access (UMA) to non-uniform memory access (\hl{NUMA}) to provide higher scalability. However, it also introduces a huge challenge to programming and compiler optimization.
Specifically, in a UMA architecture like a GPU, a program assumes that all data is accessed from a uniform memory space, with only need to partition computation to parallel processors. In contrast, a NUMA architecture forces the program to determine both computation partitioning and data placement across a distributed memory space, making it significantly more complex to program and optimize.
Given such a challenge, the existing approach is either to place all necessary data in the local memory space ~\cite{}, which could cause many data duplication across cores; or to create a global virtualized shared memory space to mimic a NUMA architecture~\cite{popart}. However, both of these approaches introduce significant memory waste or even communication overhead, limiting their effective support for real models.

In this paper, we present \oursys{}, a deep learning compiler to schedule tensor placement and transmission across distributed on-chip memory with efficient space utilization.
\oursys{} is motivated by our observation of the unique pattern of DNN workloads: the dominant operations, such as matrix multiplication or convolution, often exhibit a regular data access pattern, which read/write consecutive data tiles from input/output tensors during computation. 
Such a regular pattern allows us to relax the requirement of a uniform memory space to hold tensors.
Specifically, we could partition a tensor into consecutive data tiles, place them into distributed memory spaces, and organize a transmission ring to rotate the tensor across multiple cores. In this way, the required data tiles can be proactively delivered to the computation core in a well-organized communication order, rather than being fetched from the off-chip memory system on demand.
This forms a new ``\textit{compute-shift}'' style of computation model for accelerators with distributed memories, which differs fundamentally from the existing ``\textit{load-compute-store}'' model (i.e., load data tiles from off-chip memory, compute, and then store the result tiles back) used in shared memory based accelerators like GPU.

% , besides for a few operators like Gather/Scatter, which exhibit random access pattern.
% This unique pattern means that a uniform memory space is not necessary for these operations, as it is usually beneficial for random memory access pattern like in Gather or Scatter operators.

However, this new computation model comes up with some unique challenges.
First, different tensors could be used by different groups of processors. We need to coordinate all tensor rotations so that the required data tiles could be delivered to each processor timely.
Second, different tensor rotating plans and different computation partitioning plans create a combinatorial optimization space. Effectively optimizing in this complex space poses a substantial challenge.
Third, as the local memory on each processor is mostly on-chip memory, the aggregated memory capacity is considerably smaller than the off-chip memory. Thus, the compiler must effectively utilize the limited memory capacity to support a model size as large as possible, without compromising on computing performance.

To address these challenges, \oursys{} first introduces a distributed tensor abstraction called \textit{RotatingTensor} (\rtensor{} in short) that can rotate its partitioned tiles across a group of processors at a configurable pace. \oursys{} provides a mechanism to align the rotating paces across different tensors for the same operator based on its computation logic and partitioning plan, so that data tiles and computation can meet at the right timing in every step.
Second, the "compute-shift" model on distributed memory architecture inherently avoids the data access competition occurred in shared memory systems, which allows \oursys{} to build a sufficiently accurate cost model by considering only the communication and computation cost. Such a cost model could guide the partitioning and rotating optimization efficiently.
Third, a \rtensor{} with different rotating configurations creates different trade-offs between the memory footprint and communication cost. \oursys{} leverages a \textit{two-staged scheduling policy} to first enumerate the Pareto-optimal trade-off points for each individual operator and then make a global memory allocation for all operators, ensuring that the entire model fits into memory with optimal performance.

We implement \oursys{} in 10K lines of code with Python, including the execution plan optimization and kernel code generation. 
We conduct our evaluation using various types of DNN models, such as CNNs, transformers, and vision transformers, with different batch sizes. These models are compiled by \oursys{} and evaluated on a real distributed memory-based accelerator - Graphcore IPU Mk2 chip, as well as its variants by configuring its available cores and memory capacity.
Our evaluation shows that \oursys{} not only outperforms state-of-the-art DNN compilers and vendor-specific libraries by up to 5.2$\times$, 
but also allows for much larger models and operator sizes.
%e.g., with up to a \todo{xxx} improvement. 
More importantly, \oursys{} is the first to provide a systematic compiler approach and optimization space for distributed memory-based accelerator architectures. 
%a comprehensive optimization space and 
% an end-to-end compilation approach for distributed memory-based accelerator architectures. 
%By leveraging such flexibility, 
\oursys{} generalizes the classic distributed matrix multiplication approach (i.e., Cannon's algorithm~\cite{cannon}) for general tensor computation with 
distributed on-chip memory architectures. We wish our systematical approach could inspire and accelerate the design of more scalable 
distributed memory-based accelerators in the future.

% Outline:
% 	• Memory becomes bottleneck for today's DNN on GPUs.
% 	• Hardware exploration to mitigate such pressure:
% 		○ Move IO pressure from memory to (on-chip) network
% 		○ New architecture: shared off-chip memory -> distributed on-chip memory + Noc?
% 		○ Examples: H100->IPU, Cerebras, etc.
% 	• Introduce fundamental challenge to programming: UMA vs NUMA
% 		○ Shared memory: random access vs distributed memory: regular access
% 		○ Capacity utilization is another critical factor
% 		○ Naïve way: UMA abstraction /waste on-chip memory capacity
% 			§ Imbalance
% 			§ Fragmented access
		
% 	• Key insights: 
% 		○ DNN computation dominated by tensor computation like Matmul and Conv
% 		○ Regular data access pattern that can be inferred from their computation logics
% 			§ Computation can be partitioned into regular tiles
% 			§ Data tiles are accessed in an consecutive order from the input tensors
% 		○ Carefully partition a computation to multiple cores and arrange a tensor to be streamlined over a group of cores, so that every core can get its required input data tiles timely, instead of proactively fetching from shared memory. 
			
% 		○ Each partitioned sub-tensor can be arranged to meet the computation task on specific core.
% 		○ Tensor partitions can be streamlined  to each core instead of fetching on demand
% 		○ Create a fundamental new scheduling space.
% 	• New challenges:
% 		○ How to guarantee the data tiles to meet computation tile at the right time steps for all cores? : RotatingTensor (rTensor)
% 		○ Different rotating pace represents different trade-off between memory and cost. How to trade-off? Parato-optimal plan set guided by cost-model
% 		○ How to allocate limited memory for all operators? 
		
% 		○ Our solution:
% 		○ Computation: RotatingTensor
% 		○ Hardware-> local memory access -> no interference -> accurate cost model: 2) partition model -> one recevive one send
% 		○ Inter-operator scheduling space
% 			§ rotate or duplicate sub-tensors -> spatial-temporal space
% 			§ Constraints: data and computation aligned on each core and in each step
% 		○ Policy
% 	• Evaluation: 
% 	• Demonstration: 
% 		○ Comparable performance for compute-intensive models
% 		○ Good for memory-intensive workloads: 
% 			§ high aggregated memory bandwidth -> speedup LLM inference
% 		○ Memory capacity -> 
% 	• Looking forward & discussion
% IPU+HBM -> capacity 


% Intro:
% Motivation & Observation:
% 	• Shared Memory vs DSM accelerators
% 	• Inefficiency of existing approach 
% 	• Our idea
% Design:
% 	• Hardware Abstraction
% 	• RotatingTensor
% 	• Mapping tensor Computation to DSM
% 		○ Spatial partitioning 
% 		○ Rotating tensor
% 		○ Align the rotating pace with computation
% 	• Scheduling Optimization
% 		○ Intra-operator space  pruning
% 		○ Cost model
% 		○ Inter-operator memory allocation
% Implementation

%%%%% another draft story
% 1. 

==> intro_new_bak2.tex <==
\section{Introduction}
\label{sec:intro}

% 1. Deep learning workloads are popular today.
% 2. Many hardware accelerators have been developed to support the increasing computation demand of deep learning workloads.
% 3. As the deep learning accelerators continue to evolve, the community is actively exploring new architectural innovations to further improve the performance of deep learning workloads.
% 4. one popular trend is introducing fast inter-core connections that allow data to be exchanged across the compute cores directly without going through the off-chip memory system.

Over the years, deep learning has made significant progress and revolutionized many disciplines, such as computer vision and natural language processing.
To support the high computational demand of deep learning workloads, many hardware accelerators have been developed~\cite{a100, h100, tpu_supercomputer, ipu2, samba, tenstorrent, wse2}.

Typically, a deep learning accelerator incorporates many parallel cores, such as streaming multi-processors (SMs) on GPUs~\cite{a100}, to provide massive computing throughput. Each core is associated with a small SRAM buffer as a scratchpad memory (e.g., shared memory in each SM in a GPU) to feed the data into the compute units.
To leverage the parallelism provided by these cores, a deep learning compiler partitions the computation into multiple pieces that can be computed independently by different cores in parallel.

While the above architecture has been the most popular in the AI chip market today, as deep learning workloads continue to evolve, the community is actively exploring new architectural innovations to further improve the performance of deep learning workloads.
One popular trend today is introducing fast inter-core connections to allow data to be exchanged across cores directly, as compared to the traditional architecture in which each core performs computation independently and relies on a global shared-memory system to synchronize data.
This architectural paradigm is not only embraced by emerging deep learning accelerators like Graphcore IPU~\cite{ipu2}, SambaNova SN10~\cite{samba}, Tenstorrent Grayskull~\cite{tenstorrent}, and Cerebras WSE~\cite{wse2}, but also integrated into the latest GPU architecture, e.g., NVIDIA H100~\cite{h100}, which adds on-chip connections among multiple SMs.

% Deep learning accelerators, such as GPUs and TPUs, are widely recognized for their exceptional computing throughput, e.g., hundreds of Tera-FLOPS facilitated by their high-performance parallel computing units like TensorCores~\cite{a100, h100, tpu_supercomputer}. This makes them ideal for handling the increasing demand for processing larger deep learning models. 
% To saturate the computing throughput, such accelerators usually require a high-bandwidth memory system, e.g., hierarchical cache layers on top of a large off-chip memory like HBM~\cite{hbm}, to feed data to the computing units in time.
% However, with the increasing computing FLOPS of the accelerator chip, the computing throughput is growing significantly faster than the memory bandwidth. As a result, the deep learning workloads quickly hit the memory bandwidth wall~\cite{}. 
% However, with the increasing computing FLOPS of TensorCore, the computation throughput is growing significantly faster than the memory bandwidth growth in recent generation of GPUs, leading the deep learning workload quickly hitting the memory wall\cite{}. 

% To alleviate the memory pressure and continue scaling up the effective computing FLOPS, one solution is to increase the on-chip memory capacity, which will improve the on-chip data reuse of the deep learning workloads and reduce off-chip memory bandwidth requirement.
% As the scaling of SRAM slows down~\cite{sram_scale_slowdown}, it becomes more difficult to enlarge the on-chip memory with the traditional memory hierarchy, which typically incorporates a centralized on-chip memory that can be accessed from multiple compute cores, such as the vector memory on the Google TPU.
% As a result, recent accelerator designs have been actively exploring innovative ways to increase the on-chip memory capacity.

% First, the on-chip memory capacity has been increasing to provide significantly higher memory bandwidth than the off-chip HBM.
% Second, fast inter-core connections are introduced to exchange data across cores directly without going through the off-chip memory system. This not only increases the effective on-chip memory capacity but also enables dataflow programming model for reduced off-chip memory bandwidth requirement (see~$\S$\ref{sec:xxx}).
% To continue scaling up the effective computing FLOPS, recent accelerator designs actively explore innovative architectural changes to alleviate memory pressure. 
% Among them, two fundamental changes are becoming a mainstream trend:
% (1) enlarging the on-chip memory capacity to provide significantly higher aggregated memory bandwidth;
% and (2) introducing fast inter-core connections that allow data to be exchanged across cores directly without going through the off-chip memory system.
% This architectural paradigm is not only embraced by an emerging set of new deep learning accelerators like Graphcore IPU~\cite{ipu2}, SambaNova SN10~\cite{samba}, Tenstorrent Grayskull~\cite{tenstorrent}, Cerebras WSE~\cite{wse2}, but also integrated into the latest GPU architectures, e.g., NVIDIA H100~\cite{h100}, by introducing an on-chip connection among the shared memory of multiple stream multiprocessors.

From the programmer's perspective, the on-chip inter-core connections enable a \textit{distributed on-chip memory} architecture, in contrast to the traditional \textit{shared-memory architecture}, as each core now has the ability to directly communicate with other cores and access other cores' private scratchpad memory.
This facilitates more flexible computing paradigms, such as a dataflow programming model where one core directly consumes the output from another core, as compared to the traditional way where each core works on distinct data chunks and synchronizes the results in a global shared memory.
% such change essentially transforms the memory architecture from uniform memory access (UMA) to non-uniform memory access (\hl{NUMA}) to provide higher scalability. 

However, the distributed on-chip memory also introduces a huge challenge to programming and compiler optimization,
and it remains an open research problem on how to best exploit this new architectural feature for deep learning workloads.
Specifically, in a shared-memory architecture like a GPU, a program assumes that all data is accessed from a unified memory space, so the compiler only needs to partition computation to parallel compute cores. In contrast, a distributed on-chip memory architecture enables the program to orchestrate both computation partitioning and data placement across the distributed memory space. %, making it significantly more complex to program and optimize.
Given such a challenge, the existing approach is either to place all necessary data in the private memory of each core, which incurs significant data duplication across cores; or to create a ``virtual global memory'' illusion to emulate a shared-memory architecture~\cite{popart}. However, both approaches introduce significant memory waste or communication overhead, and they still cannot fully exploit the potential benefit of the new architecture (see $\S$\ref{sec:limit_existing_approach}).

Thus, we are motivated to revisit the compiler design for the new distributed on-chip memory architecture.
In this paper, we present \oursys{}, a deep learning compiler that exploits the benefits of such architecture by scheduling tensor placement and transmission across distributed on-chip memory. % with efficient space utilization.
\oursys{} is driven by two major observations.

First, since most DNN workloads have deterministic computation patterns, they are intrinsically a good fit for the distributed on-chip memory architecture, which provides the flexibility for the software to explicitly manage data movement between cores.
The dominant operations in a DNN model, such as matrix multiplication or convolution, often exhibit a regular data access pattern, which read/write consecutive data tiles from input/output tensors during computation. 
This allows us to relax the requirement of a unified memory space to place tensors.
Specifically, we can partition a tensor into consecutive data tiles, place them into the local memory spaces of the cores, and organize a transmission ring to \textit{rotate} the tensor across multiple cores. The required data tiles can be proactively delivered to the computation core in a well-organized communication order, rather than being fetched from a shared memory space on demand.
% \oursys{} is motivated by our observation of the unique pattern of DNN workloads: 
This forms a new ``\textit{compute-shift}'' computation model with distributed memories, which differs fundamentally from the existing ``\textit{load-compute-store}'' model (i.e., load data tiles from the global memory space, compute, and then store the result tiles back) used in shared-memory-based accelerators like GPUs.
% , besides for a few operators like Gather/Scatter, which exhibit random access pattern.
% This unique pattern means that a uniform memory space is not necessary for these operations, as it is usually beneficial for random memory access pattern like in Gather or Scatter operators.

Second, the high-speed inter-core connections enable us to better utilize the limited on-chip memory capacity.
% As the local memory on each core is on-chip SRAM, the aggregated on-chip memory capacity (usually hundreds of MBs per chip) is considerably limited compared to a globally shared memory, which is typically backed by the off-chip HBM memory (tens of GBs per chip).
In the traditional shared-memory architecture, since one core cannot access the local memory of another core, all cores may need to read the same data into their local memories, which leads to significant memory waste.
As the inter-core connections allow different cores to exchange data, we do not have to store the same data on all cores anymore.
%, since one core can effectively access another core's local memory.
The compiler can leverage this ability to better utilize the limited on-chip memory capacity rather than duplicating the data on every core.
Furthermore, as all cores can access any other core's local memory, we do not need a global on-chip memory that can be accessed by all cores (like the L2 cache in a GPU) anymore. This implies the extra hardware budget can be used more efficiently elsewhere, such as for increasing the local memory capacity for each core. In fact, this has been a common design choice for distributed on-chip memory-based accelerators such as Graphcore IPU.

Despite the potential benefits of the new architecture, the new ``compute-shift'' computation model also introduces unique challenges for the compiler.
First, different tensors could be used by different groups of cores. The compiler needs to coordinate all tensor rotations so that the required data tiles can be delivered to each core timely.
Second, different tensor rotating plans and computation partitioning plans create a combinatorial optimization space, which poses a substantial challenge for us to efficiently explore this complex space.
Third, even though the inter-core connections allow us to eliminate data duplication across cores, there will still be communication overhead for one core to fetch data from another core. Instead of having no duplication, the compiler should carefully decide how much duplication is the most appropriate to balance inter-core communication overhead and on-chip memory pressure.
% as the local memory on each core is on-chip SRAM, the aggregated on-chip memory capacity (usually hundreds of MBs per chip) is considerably limited compared to a globally shared memory, which is typically backed by the off-chip HBM memory (tens of GBs per chip). As the inter-core connections allow different cores to exchange data, the compiler should leverage this ability to better utilize the limited on-chip memory capacity rather than duplicating the data on every core.
% to support a model size as large as possible, without compromising computing performance.

To address these challenges, \oursys{} first introduces a distributed tensor abstraction called \textit{RotatingTensor} (\rtensor{} in short) that can rotate its partitioned tiles across a group of cores. % \hl{at a configurable pace}.
\oursys{} provides a mechanism to align the rotating paces of different tensors in the same operator based on its computation logic and partitioning plan, so that data tiles and computation can meet at the right timing in every step.
Second, the ``compute-shift'' model on the distributed on-chip memory architecture inherently avoids the data access competition in shared-memory systems, which allows \oursys{} to build an accurate cost model by considering only the communication and computation cost.
Such a cost model can guide the partitioning and rotating optimization efficiently.
Third, an \rtensor{} with different rotating configurations creates different trade-offs between the memory footprint and communication cost.
Such trade-offs are best exploited with operator fusion, i.e., fitting multiple operators into the on-chip memory to exploit inter-operator data reuse with the high on-chip memory bandwidth.
\oursys{} leverages a \textit{two-staged scheduling policy} to explore such trade-offs: (1) it enumerates the Pareto-optimal trade-off points for each individual operator; (2) it selects the appropriate trade-off point for each operator to generate a memory allocation plan to fit multiple operators (or even the entire DNN model) into the on-chip memory.
% Then, it makes a global memory allocation plan for all operators, ensuring that the entire model fits into memory with optimal performance.

We implement \oursys{} in 10K lines of code with Python, including the execution plan optimization and kernel code generation. 
We evaluate \oursys{} using various DNN models, such as CNNs, transformers, and vision transformers, with different batch sizes. These models are compiled by \oursys{} and executed on a real distributed memory-based accelerator - Graphcore IPU Mk2 chip, as well as its variants by configuring its available cores and memory capacity.
As the IPU chip is not backed by off-chip memory, \oursys{} will attempt to fit the entire DNN model into the on-chip memory.
Our evaluation shows that \oursys{} not only outperforms state-of-the-art DNN compilers and vendor-specific libraries by up to 5.2$\times$, 
but also allows for much larger models and operator sizes.
%e.g., with up to a \todo{xxx} improvement. 
More importantly, \oursys{} is the first to provide a systematic compiler approach and optimization space for distributed on-chip memory-based accelerators. 
%a comprehensive optimization space and 
% an end-to-end compilation approach for distributed memory-based accelerator architectures. 
%By leveraging such flexibility, 
\oursys{} generalizes the classic distributed matrix multiplication approach (i.e., Cannon's algorithm~\cite{cannon}) for general tensor computation with distributed on-chip memory architectures.
We wish our systematic approach could inspire and facilitate the design of future distributed memory-based accelerators.

% Outline:
% 	• Memory becomes bottleneck for today's DNN on GPUs.
% 	• Hardware exploration to mitigate such pressure:
% 		○ Move IO pressure from memory to (on-chip) network
% 		○ New architecture: shared off-chip memory -> distributed on-chip memory + Noc?
% 		○ Examples: H100->IPU, Cerebras, etc.
% 	• Introduce fundamental challenge to programming: UMA vs NUMA
% 		○ Shared memory: random access vs distributed memory: regular access
% 		○ Capacity utilization is another critical factor
% 		○ Naïve way: UMA abstraction /waste on-chip memory capacity
% 			§ Imbalance
% 			§ Fragmented access
		
% 	• Key insights: 
% 		○ DNN computation dominated by tensor computation like Matmul and Conv
% 		○ Regular data access pattern that can be inferred from their computation logics
% 			§ Computation can be partitioned into regular tiles
% 			§ Data tiles are accessed in an consecutive order from the input tensors
% 		○ Carefully partition a computation to multiple cores and arrange a tensor to be streamlined over a group of cores, so that every core can get its required input data tiles timely, instead of proactively fetching from shared memory. 
			
% 		○ Each partitioned sub-tensor can be arranged to meet the computation task on specific core.
% 		○ Tensor partitions can be streamlined  to each core instead of fetching on demand
% 		○ Create a fundamental new scheduling space.
% 	• New challenges:
% 		○ How to guarantee the data tiles to meet computation tile at the right time steps for all cores? : RotatingTensor (rTensor)
% 		○ Different rotating pace represents different trade-off between memory and cost. How to trade-off? Parato-optimal plan set guided by cost-model
% 		○ How to allocate limited memory for all operators? 
		
% 		○ Our solution:
% 		○ Computation: RotatingTensor
% 		○ Hardware-> local memory access -> no interference -> accurate cost model: 2) partition model -> one recevive one send
% 		○ Inter-operator scheduling space
% 			§ rotate or duplicate sub-tensors -> spatial-temporal space
% 			§ Constraints: data and computation aligned on each core and in each step
% 		○ Policy
% 	• Evaluation: 
% 	• Demonstration: 
% 		○ Comparable performance for compute-intensive models
% 		○ Good for memory-intensive workloads: 
% 			§ high aggregated memory bandwidth -> speedup LLM inference
% 		○ Memory capacity -> 
% 	• Looking forward & discussion
% IPU+HBM -> capacity 


% Intro:
% Motivation & Observation:
% 	• Shared Memory vs DSM accelerators
% 	• Inefficiency of existing approach 
% 	• Our idea
% Design:
% 	• Hardware Abstraction
% 	• RotatingTensor
% 	• Mapping tensor Computation to DSM
% 		○ Spatial partitioning 
% 		○ Rotating tensor
% 		○ Align the rotating pace with computation
% 	• Scheduling Optimization
% 		○ Intra-operator space  pruning
% 		○ Cost model
% 		○ Inter-operator memory allocation
% Implementation

%%%%% another draft story
% 1. 

==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}



%\subsection{Observation}
%\label{sec:observation}


\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/ipu-SaveSpace.drawio.pdf}
    \vspace{-3ex}
    \caption{Improve on-chip memory usage on DSM hardware.}
    \label{fig:save_mem}
    \vspace{-2ex}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.76\linewidth]{figures/motiv_mem_duplicate.pdf}
    \vspace{-3ex}
    \caption{Data duplication ratio of various operators on IPU.}
    \label{fig:ipu_mem_duplication}
    \vspace{-2ex}
\end{figure}


\noindent
\textbf{Inefficiency caused by shared-memory abstraction.}
Owing to the ease of programming, existing libraries~\cite{popart} and compilers~\cite{ansor,roller} optimize for DSM-based accelerators by abstracting their distributed memory into a virtual shared global memory, thereby creating a 2-layered memory hierarchy in conjunction with the remaining local memory. 

For instance, Graphcore's official toolchain, PopART~\cite{popart}, allocates a portion of memory in each core and abstracts it as a virtual global memory, as depicted in \Cref{fig:save_mem}(a) \cite{ipu_program}. All tensors, including persistent weights (e.g., from idle operators) and temporary activations (e.g., from active operators), are placed in the virtual global memory. 
\hl{Thus, the size of virtual global memory is equal to the total size of the DNN workload.}
During execution, each core retrieves the required data from the global space to its remaining local memory and subsequently performs local computation using only the fetched data. Given that a large portion of local memory is reserved for the virtual global memory, the local memory can only accommodate a very small sub-operator size, resulting in a significant inefficiency in computation density and increased communication overhead due to frequent data fetching from the global memory.

More critically, as a library, PopART struggles to determine the sub-operator size that can fully utilize the remaining local memory. It either generates a smaller operator size, leading to underutilization of memory (illustrated by the empty portion in \Cref{fig:save_mem}(a)), or an excessively large size that causes out-of-memory issues (\Cref{sec:eval_e2e_perf}). While compilers like Roller address this problem by searching for the maximum sub-operator that fits into the remaining memory (\Cref{fig:save_mem}(b)) \cite{roller}, the large global memory remains the fundamental factor causing inefficient usage of on-chip memory.

\hl{First, the presence of virtual global memory limits the capacity left for the local memory on each core. This limits the sub-operator size on each core, leading to low operational intensity. Even worse, due to the limited local memory size, the cores need to frequently fetch data from other cores, which leads to high inter-core communication overhead.}
\hl{Second, previous tools using virtual global memory suffer from significant memory access imbalance among different cores. This is because data in one global memory partition may be accessed more frequently than other partitions, so some cores need to serve more global memory accesses than other cores during a gather-scatter communication. As a result, the most stressed core will bottleneck all other cores.}
\hl{Third, the data needed by one core may be fragmented into different cores in the virtual global memory. This means the core must fetch data from multiple other cores, which causes significant communication overhead.}

\hl{To address these limitations, we aim to replace the global memory abstraction with the spatial-temporal mapping (\S\mbox{\ref{sec:design:space}}), which improves both computation and communication efficiencies by enabling larger sub-operator sizes and balancing inter-core communication volumes.}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/ipu-motivation_example.drawio.pdf}
    \vspace{-2ex}
    \caption{Fit operator into cores with limited capacity using shift, assuming each core can hold 11 square elements.}
    \label{fig:motivation_example}
    \vspace{-2ex}
\end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/ipu-shape_example.drawio.pdf}
    \vspace{-2ex}
    \caption{Trade-off between different partition plans.}
    \label{fig:shape_example}
    \vspace{-4ex}
\end{figure}


\vspace{0.2em}
\noindent
\textbf{Inefficiency caused by data duplication.}
Apart from the memory reserved for virtual global memory, when a core requires data from the global memory (i.e., located on another core), it duplicates the data in its local memory. This results in the actual data size stored in on-chip memory being significantly larger than the operator's tensor size. Such duplication may prevent a model from fitting onto the chip even if its size is smaller than the on-chip capacity. According to our measurements of some typical DNN operators (\Cref{fig:ipu_mem_duplication}), a large operator may consume up to 5 times the on-chip memory compared to its total variable size on IPU. This implies that more than 80\% of the on-chip memory is utilized for duplicated data for individual operators, in addition to the space reserved for virtual global memory.


% \subsection{Data duplication on DSM hardware}
% \label{sec:motivation:data_duplication}




% % While we want to place more data into the chip to enable more chip-level data reuse, we observe that the on-chip memory of DSM accelerators is inefficiently used due to data duplication.
% % In \Cref{fig:bsp}, when one core demands data from other cores, it will duplicate and store the data in its own local memory.
% % Thus, at this moment the data size occupying the on-chip memory is larger than the total data size of the tensor operators' inputs and outputs.
% % Such behavior prevents more operators from fitting into the chip even if the total sizes of their variables are smaller than the on-chip capacity, causing data swaps on the limited off-chip bandwidth, which harms the overall performance under data idleness.




% \subsection{Increasing Sub-operator Sizes}
% \label{sec:motivation:global_overhead}


% % Due to the current prosperity of GPU community, many DSM vendors build toolchains  compilation frameworks and development tools have been developed for the GPU-like architecture \cite{tvm,ansor,nnfusion,roller}.
% % Thus, to minimize programming efforts, some DSM hardware producers build development tools for their hardware by applying the ideas of existing GPU tools \cite{popart, wse2}.
% % While a global on-chip memory shared by all cores does not exist on DSM hardware, it is an important assumption for GPU programming and optimization.
% % To apply the algorithms developed for GPUs to DSM hardware, a virtual global memory is abstracted by software to hold the data shared by many cores.

% Meanwhile, due to the current prosperity of GPU community, developers attempt to optimize DSM performance following GPU optimization techniques~\cite{ansor,roller}.
% % While a global on-chip memory shared by all cores does not exist on DSM hardware, it is an important assumption for GPU programming and optimization.
% To apply the algorithms developed for GPUs to DSM hardware with minimal programming efforts, a virtual unified global memory is abstracted by software to hold the data shared by many cores, which also help reduce the duplication described above at high performance cost.

% For example, Graphcore IPU's official toolchain, PopART, reserves a portion of memory on each core and treat their combination as virtual global memory, as shown in \Cref{fig:save_mem}(a) \cite{ipu_program}.
% Both the stored parameters for future operators that are currently idle and the variables shared by multiple cores in current operator will be placed in the global memory.
% Under the DSM programming model described in \Cref{sec:background:inter_core_sync}, each core fetches the data needed in its next sub-operator from the global space to its remaining local memory during data transfer phase.
% Next, each core executes a sub-operator using the data just fetched during compute phase, while keeping the data in its portion of global memory untouched.

% In this way, data shared by different cores is spread across the global memory, so it does not have to concurrently exist on all cores that demand it. 
% To reduce memory consumption or fit the sub-operator into remaining per-core memory, a core may fetch only a small portion of the data each time, at the cost of extremely small sub-operators. 
% Thus, the reduced available size prevents us from enlarging sub-operator size for less inter-core data transfer and higher FLOPS.

% Meanwhile, PopART selects the size of sub-operators (i.e., the work done on each core per round) based on some black box heuristics. 
% In some cases, PopART generates sub-optimal sub-operators that cannot fully utilize the memory in each core, as shown by the empty portion in \Cref{fig:save_mem}(a).
% In other cases, PopART just runs out of the memory when the arbitrary size it desinate is too large, as observed later in \Cref{sec:eval_e2e_perf}.
% State of the art (SOTA) compilers supporting IPU like Roller partially address the issue by search for the maximum sub-operator that fits into the remaining memory, as shown in \Cref{fig:save_mem}(b) \cite{roller}.
% However, the large virtual global memory still bounds its potential.
% Thus, we aim to enable DSM hardware to work without global memory.





==> overview.tex <==
\section{System Design of \pname{}}
\label{sec:design}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/ipu-Copy8.drawio.pdf}
    \vspace{-2ex}
    \caption{\pname{} overview \todo{change sec after finalizing paper structure}.}
    \label{fig:overview}
    \vspace{-2.5ex}
\end{figure*}

By incorporating the above ideas, we introduce \pname{}, a compiler designed to optimize end-to-end DNN model execution on DSM-based accelerators. The workflow of \pname{} is illustrated in \Cref{fig:overview} and consists of the following steps:
1) \pname{} accepts a complete DNN model as input and generates a spatial-temporal optimization space for each operator (\S\ref{sec:design:space}).
2) For each operator, \pname{} optimizes its partitioning plan by pruning invalid options and selecting a range of optimal plans with varying memory requirements, guided by a cost model (\S\ref{sec:design:intra_op}).
3) An inter-operator memory reconciliation process is employed to determine the best end-to-end plan by deciding on appropriate active and idle memory spaces (\S\ref{sec:design:inter_op}).
4) The chosen plan is translated into a concrete program and further compiled onto accelerators like IPUs using three abstracted device interfaces (\S\ref{sec:design:hardware}).
Together, \pname{} enables efficient DNN model execution on DSM-based accelerators by optimizing both intra- and inter-operator scheduling.


% To optimize the end-to-end DNN model execution on IPU and other accelerators with DSM, we propose \pname{}, an automatic compiler that unleashes their full potential. 
% We show \pname{} components as the blue blocks in \Cref{fig:overview}.
% \begin{itemize}[leftmargin=*]
%     \item \pname{} defines a new optimization space introduced by the trade-off between memory and data transfer.
%     \item \pname{} enforces constraints to prune the large space and search for valid execution plan candidates and applies an efficient cost model to filter out a set of top plan candidates for each operator in the model.
%     \item \pname{} employs a co-evaluation mechanism to identify the optimal combination of execution plans, one for each operator, to optimize for end-to-end performance.
%     \item \pname{} overcomes hardware limitation on shift to convert an end-to-end plan into executable kernel code.
% \end{itemize}

% change spacing around display math
% \makeatletter
% \g@addto@macro\normalsize{%
%   \setlength\abovedisplayskip{10pt}
%   \setlength\belowdisplayskip{10pt}
%   \setlength\abovedisplayshortskip{10pt}
%   \setlength\belowdisplayshortskip{10pt}
% }
% \makeatother

\subsection{Spatial-Temporal Mapping Space}
\label{sec:design:space}
To map a computation, such as a DNN operator, across distributed cores, \pname{} uses a standard tensor expression to represent the operator, as described in TVM~\cite{tvm}. The expression defines the logic how each output tensor element is computed based on the input tensor values. For instance, a matrix multiplication of tensors $A$ and $B$ into $C$ expresses as follows,
\[C[m, n] \mathrel{+}= A[m, k] * B[k, n],\]
where $m$, $n$, and $k$ represent the dimension variables in both input and output tensors. The expression indicates that any value in $C$ indexed by $m$ and $n$ (e.g., $C[m, n]$) is calculated by a sum reduction over $A[m, k]$ and $B[k, n]$ for all potential indices $k$.

\hl{Similarly, \pname{} supports all operators that can be written as a tensor expression described in TVM. For example, a 2D convolution is expressed as}
$O[B, OC, OH, OW] += I[B, IC, OH+KH, OW+KW] * C[OC, IC, KH, KW]$\hl{, where B is batch size, IC/OC is input/output channel, OH/OW is output height/width, and KH/KW is kernel height/width.}

To map one operator to all cores, the tensors are partitioned across the cores and a sub-operator is composed for each core with data dependencies only on the sub-tensors assigned to it. To achieve this, \pname{} organizes all cores in a spatial-temporal space and maps all tensor partitions into it.


\vspace{0.2em}
\noindent
\textbf{Spatial mapping.}
\pname{} begins by extracting all unique dimensions present in a given tensor expression and placing them into a dimension set $S$. For example, in the matrix multiplication expression mentioned earlier, $S=\{m, n, k\}$.
If a tensor dimension is a combination of other dimensions, \pname{} selects the largest dimension to represent it. For instance, in the 1D convolution expression $O[n] += I[n + k] * C[k]$, the dimension of tensor $I$ is the sum of $n$ and $k$, with $k$ representing the kernel dimension and usually being significantly smaller than $n$ (i.e., input size). As a result, we use $n$ to represent this dimension and the dimension set becomes $S=\{n, k\}$.

To map an operator to all distributed cores, we can partition the computation along any dimensions in $S$. We use a vector of factors $F=(f_0, f_1, ..., f_n)$ to indicate the partitioning factor for each corresponding dimension in $S$. As a result, the total number of partitions is the product of all factors in $F$.
\hl{For example, a partitioning factor $F = (3, 2)$ will slice an operator with $S=\{n, k\}$ into 3*2=6 sub-operators, each of which has $S_{sub}=\{{n\over3}, {k\over2}\}$.}
We also reorganize all cores into a multi-dimensional array of shape $F$, so that each core stores one partition of the operator.
Specifically, both the input and output tensors are partitioned along $F$ and mapped to the corresponding cores. If a \hl{partitioned} dimension does not belong to a specific tensor, \pname{} automatically duplicates this tensor to all cores along this dimension.
For example, in Figure~\ref{fig:motivation_example}(b), the input tensor is partitioned along $m$, and the weight tensor lacks an $m$ dimension. Therefore, \pname{} duplicates the weight tensor along the $m$ dimension on both core 0 and core 1.
Note that if a reduction dimension\footnote{\hl{A reduction dimension is a dimension along which the input values will be reduced/summed into one output value.}} is partitioned, the result tensor will be duplicated along \hl{this partitioned} dimension on multiple cores, with each holding a partial reduction result.
Once the mapping is complete, each core holds a sub-operator that operates on only the local sub-tensors assigned to it, while still following the original computation logic.



\vspace{0.2em}
\noindent
\textbf{Temporal mapping.}
Once the spatial mapping is done, some sub-tensors may be duplicated across multiple cores to ensure local access. To address the capacity waste caused by duplication, \pname{} introduces an orthogonal partitioning mechanism called \textit{temporal mapping}, which allows a tensor to be partitioned over a group of cores and arranged in a circular ring that shifts its partitions in multiple time steps.

In temporal mapping, a tensor $T$ can be tiled along one of its dimensions over $N$ cores with a partition factor $f$. When $f=N$, the tensor is evenly partitioned into $N$ parts and forms a full shift ring to be shared over the $N$ cores in $N-1$ steps, as depicted in Figure~\ref{fig:shift}(c). If $f<N$ (assuming $f$ divides $N$), every $f$ cores will form a local shift ring, resulting in a total of $N/f$ rings. This means the tensor $T$ is duplicated in each ring for a total of $N/f$ time, as illustrated in Figure~\ref{fig:shift}(b). In an extreme case where we specify $f=1$, tensor $T$ is duplicated on every core, requiring zero shift steps, as shown in Figure~\ref{fig:shift}(a). This is also the default case after spatial mapping.

Temporal mapping differs from spatial mapping in that it can be specified individually for each tensor. 
Thus, a vector of partition factors, denoted as $F_t=(f_0, f_1, ..., f_d)$, can be further defined for each tensor for each temporal dimension, with each factor corresponding to a particular tensor dimension. 
In practice, it suffices to only perform temporal mapping for duplicated tensors to prevent unnecessary shift steps.

In light of this, \pname{} introduces a comprehensive operator partition space for distributed cores along both \hl{spatially and temporally partitioned dimensions}.
\hl{An operator will first be spatially partitioned to generate a set of spatial mapping plans. For each spatial mapping plan, a set of temporal partitioning factors can be further defined for each tensor, with each factor corresponding to a particular tensor dimension.}
A distinct partitioning plan is uniquely established by a spatial factor vector $F_s$ and multiple temporal factor vectors $F_t^i$ for each tensor $i$.
Each valid partitioning plan implies a unique execution plan that covers the mapping of each tensor to individual cores, the flow of sub-tensors across cores, and the computation of each core at a given step.
For example, if we specify the $F_s=(m:N, k:1, n:N)$, $F_t^{out}=(m:1, n:1)$, $F_t^{in0}=(m:1, k:N), F_t^{in1}=(k:N, n:1)$ for a matrix multiplication $C=A*B$, it will automatically form an $N\times N$ Cannon's algorithm~\cite{cannon} for distributed matrix multiplication, as illustrated in Figure~\ref{fig:cannon}(a).
\hl{Since \pname{} homogeneously partitions an operator across all cores, each sub-operator has exactly the same computation and communication pattern. By keeping the workloads on all cores balanced, \pname{} prevents the performance from being bottlenecked by slower threads.}

% \yiqi{for matmul(m, k, n) with output stationary cannon, $F_s=(m:N, k:1, n:N)$, \\
% $F_t^{out}=(m:1, n:1)$, $F_t^0=(m:1, k:N), F_t^1=(k:N, n:1)$}


% To generate the execution plans for one operator, we first partition the operator into spatial parts as shown in \Cref{fig:motivation_example}b, where each part is mapped to one core.
% After that, we further partition the resulting sub-operators into temporal rounds as shown in \Cref{fig:motivation_example}c.

% To abstract the above partitions, we develop the terminology shown in

% $\\$OP info:\\
% \yiqi{dim\_lengths}
% \\$[chl=dim0\_len, ker\_wid=dim1\_len, ...]$\\
% \yiqi{variable\_shapes}
% \\$[tensorA: [[chl\_idx], [ker\_wid\_idx, out\_wid\_idx]], \\
% tensorB: [[...], [..., ...], [...]]]$

% $\\$Partition info:\\
% \yiqi{num\_spatial\_partitions}
% \\$[dim0\_parts, dim1\_parts, dim2\_parts]$\\
% \yiqi{num\_temporal\_partitions}
% \\$[dim0: [tensorA\_parts, tensorB\_parts, tensorC\_parts], \\
% dim1: [tensorA\_parts, tensorB\_parts, tensorC\_parts], \\
% dim2: [tensorA\_parts, tensorB\_parts, tensorC\_parts]]$

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/ipu-factor.drawio.pdf}
    \vspace{-2.5ex}
    \caption{Illustration of temporal mapping.}
    \label{fig:shift}
    \vspace{-2ex}
\end{figure}

\subsection{Cost-aware Intra-operator Scheduling}
\label{sec:design:intra_op}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/ipu-cannon.drawio.pdf}
    \vspace{-3ex}
    \caption{Cannon Algorithm.}
    \label{fig:cannon}
    \vspace{-3.5ex}
\end{figure}

Although the aforementioned mechanism is flexible to represent all possible partitioning plans, it presents a substantial optimization space that contains numerous configurations that are either invalid or noticeably inefficient. To address this issue, \pname{} applies some explicit optimization rules as constraints during the partitioning process.  
For example, coordinating the shift of multiple tensors can lead to substantial savings in terms of both data transfer volume and computation steps. 
\hl{\pname{} first uses the constraints to filter out partitioning plans that are highly possible to be ineffective, which reduces search space size and speeds up compilation.}
To this end, we have divided our constraint rules into three categories: spatial parallelism constraints, temporal alignment constraints, and computation padding constraints. 
\hl{Then, \pname{} uses a cost model to find the optimal plans that require the least memory capacity or execution time.}

\vspace{0.2em}
\noindent
\textbf{Parallelism constraints.}
To better align with the partition size of an operator, \pname{} allows an operator to be mapped on a subset of cores, so the total number of spatial partitions in a partitioning plan could be less than the total number of available cores. 
However, utilizing too few cores for an execution plan could lead to significant inefficiencies. 
Thus, we also enforce a constraint on the ratio of idle cores, ensuring that it is less than a specified threshold, such as 5\%.

\hl{In practice, the parallelism constraint threshold can be configured by users, and \pname{} automatically relaxes the threshold for operators with no qualified plans under the given threshold. In our experiments, we set the threshold to 5\% to filter out plans utilizing less than 95\% of the cores. For small operators that cannot saturate 95\% of the cores, \pname{} will iteratively double the threshold until it finds a plan, as these small operators are rare and incur low execution overhead. This allows \pname{} to efficiently find promising plans.}


\vspace{0.2em}
\noindent
\textbf{Alignment constraints.}
To ensure that a temporal partitioning can be translated into a valid execution plan, the product of the temporal partition factors of a tensor (i.e., the total number of temporal partitions) should be a factor of the replication number caused by spatial partitioning. 
Additionally, for different tensors of an operator that share a common dimension, all their temporal factors on this dimension should be aligned. 
Thus, any pair of temporal factors should be a factor or multiple of each other. 
This approach allows each tensor or sub-tensor to flow across cores at a different pace, while ensuring that corresponding tensor partitions can meet at the same time step on a specific core.

For instance, consider the variant Cannon matrix multiplication illustrated in Figure~\ref{fig:cannon}(b), where tensor B has a temporal partitioning along dimension $k$ for an $N/2$ factor (i.e., $F_s=(N, N)$, $F_t^0=(1, N)$, and $F_t^1=(N/2, 1)$). As a result, tensor B is duplicated twice and shifted once every two time steps, while tensor A is still shifted for each step.

%\yiqi{The above scenario partitions one shift dimension with length $N$ into two shift dimensions with lengths $N/2$ and $2$. Thus, we can choose from two nested loop options with either of the shift dimensions being the outer loop. On execution, both tensors shift one step per iteration transition of the $N/2$ loop, while only tensor A shifts one step per iteration transition of the loop with length $2$, as shown in \Cref{fig:overview}(b)}

\vspace{0.2em}
\noindent
\textbf{Computation padding constraints.}
In order to take advantage of the fast matrix unit present in each core, such as the AMP in IPU, it is often necessary to pad the matrix shape of a sub-operator to a multiple of the matrix unit size. However, if a partitioning plan leads to a sub-operator shape that requires too much padding, significant amount of wasted computation occurs. Thus, \pname{} restricts the padding size to be within a small ratio when compared to its tensor size.

\hl{The padding constraint is a common practice for DNN compilers\mbox{~\cite{roller,tensorir}}. T10 leverages a similar approach by exposing the constraint to the user as a tunable compiler hyper-parameter. A smaller padding constraint helps quickly filter out inefficient partitioning plans, while a larger padding constraint includes more opportunities to find better partitioning plans at a cost of longer compilation time.
In our experiments, we use a default value that allows at most 25\% padding size compared to the tensor size. If a very small operator has no plans that saturate 75\% of the SIMD width, T10 iteratively doubles the padding constraint until it finds a plan.}



% \yiqi{Product of temporal\_parts per tensor for all dims is a factor of its number of replicas. (e.g., 8 cores cannot evenly hold 7 pieces)}

% \yiqi{The temporal\_parts per dim for all tensors must be factor or multiple of each other. (e.g., dividing 2 tensors along the same dim into 3 and 4 pieces respectively will result in unaligned shifts)}



\vspace{0.2em}
\noindent
\textbf{Plan selection guided by cost model.}
After applying the constraints mentioned above, there still remain a significant number of valid mapping plans for each operator. Thus, \pname{} further selects the optimal candidate plans by taking advantage of the unique feature of DSM-based architecture, which allows for the easy derivation of an accurate cost model. This is due to the inherent execution patterns that facilitate accurate performance prediction. Specifically, the explicit separation of computation and communication phases in the execution model, such as BSP, allows for the natural modeling of the overall latency independently. Furthermore, the computation on each core in each execution step only consumes data from local memory, which inherently prevents unpredictable memory stall behaviors from lower-level memory. In the communication phase, the time taken for data transfer is highly related to the transfer volume, which can be easily modeled by a linear regression model for a specific accelerator. Lastly, the synchronization overhead at each iteration is deterministic and relatively short compared to computation and communication time. Based on these observations, we can estimate the memory utilization and execution time for each plan. Specifically, the memory consumption is equivalent to the sub-tensor size, which can be directly inferred given a partition plan. For the computation time of a sub-operator, we default to fitting a linear regression model that takes the total flops of a sub-operator as a variable for each operator type. For some special operator implementations, we extend the regression model by adding more critical factors such as tensor size and number of loops. We also expose an interface for users to implement a custom cost function for custom kernels. 
Using the cost model, \hl{T10 analyzes the sub-operator size and execution time for each operator given a specific partitioning plan.}
It can efficiently examine each valid plan and choose the best candidates that sits in the best memory and execution time trade-off line, as illustrated by the green points in Figure~\ref{fig:overview}(b).

\subsection{Inter-operator Memory Reconciliation}
\label{sec:design:inter_op}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/ipu-idle.drawio.pdf}
    \vspace{-1.5ex}
    \caption{Deduplicate idle operators.}
    \label{fig:idle}
    \vspace{-3ex}
\end{figure}

DSM accelerators usually have sizable on-chip memory but comparatively limited off-chip memory bandwidth. 
\hl{Meanwhile, the data sharing between adjacent operators is very frequent, as many operators take the output of the preceding operator as input. In fact, one benefit of DSM-based accelerators over GPUs is that its large on-chip memory can fit a chain of operators, so the adjacent operators can share data on chip. On the contrary, the GPU often cannot even fit one single operator in its on-chip memory, so adjacent operators can only exchange data through the slow off-chip memory.
}
To execute a complete DNN model, \pname{} follows the common approach which fits all operator parameters of the model into the on-chip memory while allocating the off-chip bandwidth solely for transferring input data and output results.

\vspace{0.2em}
\noindent
\textbf{Idle and active operator state.}
For each operator, \pname{}'s intra-operator scheduling can generate multiple optimal plans, each representing a different trade-off between memory consumption and execution latency. For example, a plan may use more memory space for storing some tensor replicas to trade off for lower latency due to fewer shifting steps. With the fast inter-core connection of DSM architecture, two partitioning plans can be assigned for each operator - one for minimum memory usage before the operator execution (called idle state) and one for fast execution time during the execution (called active state). 
When an operator begins to execute, a warm-up phase transforms the partitioning plan from idle state to active state, i.e., by transferring the necessary data through the inter-core connection. Figure~\ref{fig:idle} illustrates a matrix multiplication operator and its different states. 
In the idle state, the partitioning plan with less duplication is chosen to save memory consumption. During the warm-up stage, a few sub-tensors are transferred to other cores to change into another partitioning plan, which involves duplicating one input tensor for multiple times but leads to faster execution time due to its zero shift step requirement.
\hl{Since both the idle and active plans are candidate plans generated by intra-operator scheduling, and they share the same spatial mapping, the only difference between the two plans is that they duplicate the tensors differently. Thus, \pname{} makes a multi-broadcast plan like the one shown in Figure\mbox{~\ref{fig:idle}} by comparing the placement of each tensor between both plans.}

\hl{Consequently, there is a trade-off between the memory usage at idle state and the overhead at warm-up phase. If the memory is very limited, data will be significantly deduplicated at idle state, and the warmup overhead can be high. Thus, \pname{} employs a holistic memory reconciliation mechanism to consider this trade-off and optimize the end-to-end execution time.}


% \begin{algorithm}[t]
% % \footnotesize
% \caption{Inter-operator memory reconciliation policy.}
% \label{alg:priority}
% \begin{algorithmic}[1]
% % \State priority\_list = [wl.priority for wl in workload\_list]
% \Function{get\_best\_idle\_configs}{[[op0\_idle\_configs], [op1\_idle\_configs], ...]}
% % https://drive.google.com/file/d/1gcI2pbnteWPXEvKO05_x6oUnLR3acn6l/view?usp=sharing   Inter OP Tradeoff
%     \State start from idle configs without duplication for all ops
%     \While{idle space < on-chip memory}
%         \For{all ops}
%             \State apply fastest exec plan w/o mem overflow
%         \EndFor
%         \State record total latency
%         \State apply config increment step with highest 
%         \State $delta(warmup\_time) / delta(idle\_mem)$
%     \EndWhile
%     \State return best\_configs with lowest total latency
% \EndFunction
% \end{algorithmic}
% \end{algorithm}

% \setlength{\textfloatsep}{7pt}
\begin{algorithm}[t]
\footnotesize
\caption{Inter-operator memory reconciliation policy.}
\label{alg:priority}
\begin{algorithmic}[1]
% \State priority\_list = [wl.priority for wl in workload\_list]
\Function{get\_best\_idle\_configs}{[[op0\_configs], [op1\_configs], ...]}
    \For{op in all\_ops}
        \State idle\_plan[op] <- plan with min memory use
    \EndFor
    \While{sum(idle\_plan[].mem) < max\_mem\_per\_core}
        \For{op in all ops}
            \State exec\_plan[op] <- fastest plan fits in mem
        \EndFor
        \State time <- estimate\_total\_time(idle\_plan, exec\_plan)
        \If{time < cur\_best\_time}
            \State cur\_best\_time <- time
            \State cur\_best\_plan <- (idle\_plan, exec\_plan)
        \EndIf
        \State increment idle plan for op with highest $-\Delta T_W /\Delta M_I$
    \EndWhile
    \State return cur\_best\_plan
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{figure*}
    \centering
    \includegraphics[page=5,width=0.9\linewidth]{figures/ipu-Placement.drawio.pdf}
    \vspace{-2.5ex}
    \caption{Sub-tensor placement for a 3$\times$3 Cannon algorithm.}
    \label{fig:placement}
    \vspace{-2ex}
\end{figure*}


\begin{figure}[t]
    \centering
    \includegraphics[page=5,width=0.9\linewidth]{figures/ipu-ComputeSet.drawio.pdf}
    \vspace{-3ex}
    \caption{IPU kernel code example.}
    \label{fig:codegen}
    \vspace{-1ex}
\end{figure}

\vspace{0.2em}
\noindent
\textbf{Holistic memory reconciliation.}
During the execution of the model, only one operator can be executed at any given time, while other operators are in the idle state and only occupy a portion of the idle memory space to store their tensors. As each operator could have different choices for the idle and active plans, a global optimization execution plan is needed to reconcile each operator's trade-off space holistically. \pname{} achieves this by deciding on an optimal memory size allocation for idle memory and active memory. Algorithm~\ref{alg:priority} presents \pname{}'s memory reconciliation process. Initially, \pname{} assigns the partitioning plan with zero duplication as the idle plan for all operators. The remaining memory space after placing all the idle operators is considered the active memory, which will be used for executing each operator. \pname{} searches for the best execution plan by greedily trading more active space for idle space, aiming to reduce more warm-up time (due to more duplication) at a cost of only slightly increasing execution time (due to fewer duplications). For each searching step, \pname{} first selects the best operator and its partitioning plan that can reduce the most warm-up time by adding the smallest idle space. This plan is found by calculating the ratio of $\Delta T_W /\Delta M_I$ for each operator, where $\Delta T_W$ and $\Delta M_I$ are the reduced warm-up time and increased idle memory space, respectively, if the next partitioning plan is chosen for an operator. After selecting the best plan, the active space is updated by subtracting $\Delta M_I$. Then, \pname{} calculates the new execution time by enumerating each operator to find the fastest execution plan that can fit in the given active memory space and accumulates its latency into the total execution latency. 
\hl{If there is no way to fit all operators, \pname{} will not find a valid end-to-end plan to report.}
Conclusively, while there are $\prod_{i=0}^{\# ops}(op[i].num\_idle\_plans)$ idle plan combinations in total, we acquire \hl{an optimized} one by searching only $\sum_{i=0}^{\# ops}(op[i].num\_idle\_plans)$ promising combinations.
Given the moderate number of possible trade-off configurations, \pname{} currently searches all steps and chooses the one that can lead to the minimum end-to-end execution time.



% For elementwise and pure-reduction OPs (overall duplication is always low for any spatial partition plans, and at least one var has all dims), do not change partition configuration if reuse.

% Due to the limited off-chip memory bandwidth of IPU and the large on-chip memory, the most common usecase of IPU is that we put the entire model parameters 
% for all operators inside the on-chip memory, while reserving the off-chip link exclusively for transferring input data and output results. 
% Thus, at any time of the execution there is only one operator being actively executed, while other idle operators still occupy the on-chip memory to store their parameters.
% However, some of the promising candidate plans we found for each operator in \Cref{sec:design:intra_op} employ a moderate amount of duplication to improve the execution FLOPS. 
% Thus, we can further deduplicate the parameters when their operators are idle to save more on-chip memory.


\subsection{Hardware Abstraction}
\label{sec:design:hardware}

% \setlength{\textfloatsep}{2em}


\noindent
\textbf{\pname{} hardware interface.}
% The optimal partitioning plan for an end-to-end model achieved by \pname{} above is a configuration intended to be mapped to general DSM-based architectures.
To facilitate adaptation to various DSM-based accelerators, \pname{} abstracts three key device interfaces: \texttt{allocate}, \texttt{compute}, and \texttt{shift}.
\texttt{allocate} serves as a compile-time interface that enables \pname{} to allocate memory space for placing tensor partitions beforehand. \texttt{compute} functions as a code generation interface that emits instructions for computing a specific sub-operator on a core. By default, \pname{} utilizes a few pre-defined code templates to generate single-core computing logic for each specific partition configuration.
Lastly, \texttt{shift} serves as a runtime communication primitive that offers a memory-efficient method for transferring a tensor from one core to another.
% Note that directly copying a tensor across cores needs a memory buffer on both the sender and receiver sides, resulting in significant waste of on-chip memory. \pname{} provides a default implementation of \texttt{shift} by dividing a tensor into sufficiently large chunks that can saturate the transferring bandwidth. The appropriate chunk size is tuned only once for a specific device.

\vspace{0.2em}
\noindent
\textbf{Sub-tensor memory allocation.}
By utilizing the above hardware interface, a concrete execution plan is generated from the partition configuration. At compile-time, \pname{} pre-allocates the entire memory space and assigns each sub-tensor to its corresponding core. To optimize memory usage, \pname{} performs a tensor liveness analysis to reuse the memory of precedent operators. To ensure that sub-tensors from different tensors are co-located in the same core at each shift step, \pname{} carefully arranges the initial placement of each tensor partition based on their dependencies with others.

As an example, the process of placing sub-tensors for a 3$\times$3 Cannon matrix multiplication is illustrated in \Cref{fig:placement}. Initially, all output sub-tensors ($C_j^i$) are allocated based on the partitioning plan. The first sub-tensor set (i.e., $A^0_0, A^0_1, A^0_2$) is then partitioned along the temporal dimension and distributed to the corresponding cores (the first row of cores). Given the current placement of $A^0_i$ and $C^0_i$, we infer that $B_i^i$ should be placed in the first row of cores due to data dependency. Subsequently, the remaining $B_i^j$ sub-tensors are placed sequentially in each column of cores. Following this process, the placement of all $A_i^j$ sub-tensors can be inferred.
% Note that such placement process is general to be applied to various partition plans.

\vspace{0.2em}
\noindent
\textbf{Sub-tensor compute scheduling.}
% After the tensors are placed, 
\pname{} arranges the computation on each core as nested loops of interleaved \texttt{compute} and \texttt{shift} stages. Each loop corresponds to a temporal partition number.
% For example, if there are two dimensions to shift, $m$ and $n$, with $m$ shifting twice and $n$ shifting once, then there are two valid 5-time shift schedules: shift(m)$\times2\to$ shift(n) $\to$ shift(m)$\times2\to$ or shift(n) $\to$ shift(m) $\to$ shift(n) $\to$ shift(m) $\to$ shift(n).
To determine the optimal loop order, \pname{} designates the dimension belonging to the tensor with the smaller size as the inner loops to reduce the total communication volume, as the inner loops are executed more times.

% During shifts, each core performs one round of computation on its local data. To generate local computations for each core, \pname{} invokes the corresponding \texttt{compute} function by taking the partition configuration and tensor expression as inputs. 



% for the shift stage,  determine the order of nested loops for all shifted dimensions. For instance, if there are two dimensions to shift, $m$ for 2 times and $n$ for 1 time, then there are two valid 5-time shift schedules: shift(m)$\times2$->shift(n)->shift(m)$\times2$ or shift(n)->shift(m)->shift(n)->shift(m)->shift(n). In practice, we designate shifts with smaller tensor sizes as inner loops to decrease the total shift volume.






\subsection{Put Them Together}
\label{sec:design:put_together}

\hl{For intra-operator scheduling, \pname{} enumerates the spatial-temporal partitioning plans for an operator as follows. First, the spatial partitioning space is determined by the available number of cores. \pname{} enumerates all spatial partitioning plans such that the number of spatial partitions is no greater than the total number of available cores. It also applies the parallelism constraint to filter out the spatial plans that use too few cores (i.e., have too few partitions). After spatial partitioning, some parts of the tensors may be duplicated across multiple cores for local access. Hence, for each spatial partitioning plan, \pname{} enumerates the corresponding temporal partitioning plans that satisfy the alignment constraint and the padding constraint. This gives a set of valid spatial-temporal partitioning plans for this operator. Then, \pname{} leverages the cost model to estimate the memory consumption and execution time of each spatial-temporal plan, and keeps only the Pareto-optimal plans.}

\hl{By combining intra and inter-operator scheduling, \pname{} aims to solve the fundamental problem on optimizing the trade-offs between memory consumption and execution efficiency for each operator, which forms a combinatorial optimization space.
The key insight in \pname{} is to use an aligned "cost-efficient metric" to unify the trade-off spaces in each individual operator. The metric defines how much latency can be reduced by giving a certain memory space for each operator. By leveraging such aligned metric, \pname{} is able to separate the problem into local optimizations and global optimizations. Locally, it generates the most cost-efficient plans of each operator under variant memory requirements. Globally, it decides which plan should be used for each operator by considering the global cost-efficiency i.e., end-to-end latency with a given memory budget. This leads to our efficient greedy memory reconciliation algorithm for navigating the large search space.}


==> revision_plan.tex <==
\onecolumn
\thispagestyle{plain}
\pagestyle{plain}

\pagenumbering{arabic}

% \setstretch{0.9}

\centerline{\LARGE \textbf{Revision Log of \pname}}
\vspace{1ex}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent {\large \hlcommon{\textbf{Common Questions}}}


% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]

\item \textbf{Discussion of Related Work}      

% Q1 Q2 \S\ref{sec:related}

We fully revise \S\ref{sec:related} to make an in-depth comparison between \pname{} and other compilers. Specifically, we compare DL compilers for shared memory, compilers for multiple devices, and compilers for dataflow architectures, and then discuss the uniqueness of \pname{}'s approach and \pname{}'s compatibility with other works.
%three types
\vspace{0.2em}


\item \textbf{Future Applicability of \pname}  

% Q3 Q7 \S\ref{sec:discussion}

We add \S\ref{sec:discussion} to discuss how techniques proposed by \pname{} benefit other scenarios, including various hardware with inter-core connections and distributed serving on interconnected chips, by optimizing memory usage and communication overhead.
%elaborate
\vspace{0.2em}



\item \textbf{Novel Research Contributions}   

% Q3 Q7 \S\ref{sec:discussion}

In \S\ref{sec:related}, we highlight the novelty of \pname{}.
%elaborate
\vspace{0.2em}



\item \textbf{Support for Operations like ReduceScatter}      

In \S\ref{sec:related}, we clarify how \pname{} differs from multi-device settings and does not rely on operations like ReduceScatter. 
\vspace{0.2em}


\item \textbf{Operator Dependency} 

In \S\ref{sec:implementation}, we add a paragraph to clarify how \pname{} handles operator dependencies.
\vspace{0.2em}



\item \textbf{Iteration Batching in LLM Inference Serving}      

In \S\ref{sec:related}, we discuss \pname{}'s compatibility with existing iteration batching works.
\vspace{0.2em}

% \item \textbf{Research Importance}

% \S\ref{sec:intro} (Hopper inter-SM)
% \vspace{0.2em}







\end{enumerate}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\noindent {\large \hlRA{\textbf{Reviewer A}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]


\item \textbf{\pname{} and Inter-chip Optimizations} 

In \S\ref{sec:discussion}, we discuss \pname{}'s implications in the inter-chip setting. 
\vspace{0.2em}


\item \textbf{Operator Representation}   

In \S\ref{sec:design:compute}, we clarify the definition of Tensor Expression.
\vspace{0.2em}



\item \textbf{Search Constraints}   

In \S\ref{subsubsec:intra-operator}, we elaborate on the search space constraints.
\vspace{0.2em}



\item \textbf{``Worst Case'' Program for \pname{}}   

In \S\ref{sec:eval_intra_op}, we clarify that the first 3 operators (Conv, MatMul, Gather) discussed in \Cref{fig:intra_search} already represent the “worst case” operators in our experiments.
\vspace{0.2em}


\item \textbf{Clarification on \pname{}'s Compilation Times}    

In \S\ref{sec:eval_intra_op}, we elaborate on \pname{}'s compilation times.
\vspace{0.2em}


\item \textbf{Tradeoff Between Compilation Time and Execution Time}    

In \S\ref{sec:eval_intra_op}, we add the discussion about the tradeoff between compilation and execution time.
\vspace{0.2em}

\item \textbf{Discussion on Triton and Mosaic}   

In \S\ref{sec:related}, we add the discussion about how \pname{} differs from Triton and Mosaic. % add friendliAI
\vspace{0.2em}


\item \textbf{Presentation of Figures}     

We fix the rendering issues for all figures and clarify the purpose of \Cref{fig:scale} in \S\ref{sec:eval_sens_vary_core_mem}.
\vspace{0.2em}

\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\noindent {\large \hlB{\textbf{Reviewer B}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]


\item \textbf{Energy Efficiency}  

In \S\ref{sec:discussion}, we discuss why inter-core connections can bring energy efficiency benefits.
\vspace{0.2em}


\item \textbf{Execution Procedure on IPU} 

In \S\ref{sec:limit_existing_approach}, we clarify the execution procedure on IPU (i.e., the IPU stores an entire model on the chip by default).
\vspace{0.2em}


\end{enumerate}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\noindent {\large \hlC{\textbf{Reviewer C}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]



\item \textbf{Search Procedure in \pname{}}  

In \S\ref{sec:eval_intra_op}, we clarify how \pname{} handles numerous candidate plans.
\vspace{0.2em}


\end{enumerate}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\noindent {\large \hlD{\textbf{Reviewer D}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]



\item \textbf{Cost Model}  

In \S\ref{subsubsec:intra-operator}, we clarify how the cost model is built in \pname{}.
\vspace{0.2em}


\item \textbf{Multi-chip Performance} 

In \S\ref{sec:eval_llm}, we clarify why we use single-chip performance to represent multi-chip performance.
\vspace{0.2em}


\item \textbf{Practicality of Combining IPU with HBM} 

In \S\ref{sec:discussion}, we discuss the practicality of attaching HBM to IPU.
\vspace{0.2em}





\end{enumerate}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\noindent {\large \hlE{\textbf{Reviewer E}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]


\item \textbf{Applicability of \pname{} to Other Architectures} 

In \S\ref{sec:discussion}, we discuss the applicability of \pname{}.
\vspace{0.2em}



\item \textbf{Comparison to the Abstractions in Roller}       

In \S\ref{sec:design}, we highlight the purpose of the rTensor abstraction. In \S\ref{sec:related}, we clarify how the abstractions in \pname{} differ from those in Roller.
\vspace{0.2em}


\item \textbf{Effective Bandwidth Achieved by \pname{}} 

We add the experimental results for the bandwidth utilizations in \S\ref{sec:eval_e2e_perf} and \Cref{fig:noc_util}.
\vspace{0.2em}



\end{enumerate}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\noindent {\large \hlF{\textbf{Reviewer F}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]

\item \textbf{Running An Entire LLM on IPUs} 

In \S\ref{sec:eval_llm}, we clarify how to run an entire LLM with multiple IPU chips, and why the single-chip performance of a few layers can reflect the performance of the entire model. 
\vspace{0.2em}

\item \textbf{IPU vs. GPU and Compute-Shift vs. VGM} 

In \S\ref{sec:discussion}, we discuss \pname{}'s benefits for the latest GPUs with inter-SM connections.
\vspace{0.2em}



\item \textbf{Inference vs. Training} 

In \S\ref{sec:design:compute}, we clarify that \pname{}'s approach supports both training and inference, as their operators can be represented as tensor expressions. In \S\ref{sec:eval_setup}, we clarify that we focused on inference in our evaluation because the current generation IPU chip employs limited on-chip memory capacity and is mostly used for inference.
\vspace{0.2em}



\item \textbf{TFLOPS Achieved by T10} 

In \S\ref{sec:eval_gpu}, we clarify why TFLOPS is not the focus of our evaluation, since most inference workloads are bounded by memory bandwidth.
\vspace{0.2em}




\end{enumerate}
